Cross-Subject Deep Transfer Models for Evoked Potentials in Brain-Computer Interface

Brain Computer Interface (BCI) technologies have the potential to improve the lives of millions of people around the world, whether through assistive technologies or clinical diagnostic tools. Despite advancements in the field, however, at present consumer and clinical viability remains low. A key reason for this is that many of the existing BCI deployments require substantial data collection per end-user, which can be cumbersome, tedious, and error-prone to collect. We address this challenge via a deep learning model, which, when trained across sufficient data from multiple subjects, offers reasonable performance out-of-the-box, and can be customized to novel subjects via a transfer learning process. We demonstrate the fundamental viability of our approach by repurposing an older but well-curated electroencephalography (EEG) dataset and benchmarking against several common approaches/techniques. We then partition this dataset into a transfer learning benchmark and demonstrate that our approach significantly reduces data collection burden per-subject. This suggests that our model and methodology may yield improvements to BCI technologies and enhance their consumer/clinical viability.

==> README <==

August 26, 2015


IEEEtran is a LaTeX class for authors of the Institute of Electrical and
Electronics Engineers (IEEE) transactions journals and conferences.
The latest version of the IEEEtran package can be found at CTAN:

http://www.ctan.org/pkg/ieeetran

as well as within IEEE's site:

http://www.ieee.org/

For latest news, helpful tips, answers to frequently asked questions,
beta releases and other support, visit the IEEEtran home page at my
website:

http://www.michaelshell.org/tex/ieeetran/

Version 1.8b has a number of significant changes over the v1.8a release.
For a full history of changes, please read the file changelog.txt.
The most notable changes in this release include:

 1) Added new comsoc mode for the IEEE Communications Society.
    This mode (at present) only invokes the use of the newtxmath math fonts.
 
 2) Revised IEEEeqnarray column specifications to work with active " 
    (or other punctuation catcode changes) as with babel under the
    german or ngerman language modes. 
    Thanks to Stefan M. Moser for reporting this problem.

 3) Added \indexspace and other index related macros as newer versions of
    article.cls now do. These macros are needed to avoid an error when
    using the glossaries package.
    Thanks to Sebastian Nyberg for suggesting this change.

 4) Fixed odd/even page header font bug under compsoc mode and
    other page style code improvements.
    Thanks to Marco Paolieri for reporting this problem.

 5) Added hooks to allow for easy control of spacing above title.

 6) Added the \IEEEnoauxwrite command.
    Thanks to Sudarshan Mukherjee for suggesting this feature.


NOTE: Take care not to confuse the "comsoc" and "compsoc" class
options/modes as they are very different:

comsoc  ==> IEEE Communications Society
compsoc ==> IEEE Computer Society

The comsoc mode requires that an acceptable Times math font be available on
the LaTeX system. This requirement will be enforced by IEEEtran in comsoc
mode. Either the freely available newtxmath font by Michael Sharpe
http://www.ctan.org/pkg/newtx
(version 1.451, July 28, 2015 or later is recommended)
or the commercial MathTime font (e.g., mtpro2.sty) is acceptable.
See Section II-D (2.4) "Class Options - comsoc, compsoc, transmag" of
the IEEEtran HOWTO for more details.


Best wishes for all your publication endeavors,

Michael Shell
http://www.michaelshell.org/


********************************** Files **********************************

README                 - This file.

IEEEtran.cls           - The IEEEtran LaTeX class file.

changelog.txt          - The revision history.

IEEEtran_HOWTO.pdf     - The IEEEtran LaTeX class user manual.

bare_conf.tex          - A bare bones starter file for IEEE conference papers.

bare_conf_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         conference papers.

bare_jrnl.tex          - A bare bones starter file for IEEE journal papers.

bare_jrnl_comsoc.tex   - A bare bones starter file for IEEE Communications
                         Society journal papers.

bare_jrnl_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         journal papers.

bare_jrnl_transmag.tex - A bare bones starter file for IEEE Transactions
                         on Magnetics journal papers.

bare_adv.tex           - A bare bones starter file showing advanced
                         techniques such as conditional compilation,
                         hyperlinks, PDF thumbnails, etc. The illustrated
                         format is for an IEEE Computer Society journal paper.

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall the IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtran.cls, IEEEtran_HOWTO.pdf, bare_adv.tex,
                   bare_conf.tex, bare_conf_compsoc.tex, bare_jrnl.tex,
                   bare_jrnl_comsoc.tex, bare_jrnl_compsoc.tex,
                   bare_jrnl_transmag.tex
***************************************************************************


==> sections/Approach-Old.tex <==
\section{Approach}\label{sec:approach}

In Sec. \ref{sec:dataset}, we describe the dataset and data splits that we use under two evaluation scenarios: performance benchmarking (Scenario 1) and transfer learning evaluation (Scenario 2). We then describe our deep learning architecture and elaborate on our design rationale (Sec. \ref{sec:dl_model}). Next, we introduce traditional models against which we benchmark, under Scenario 1 to establish the viability of our deep learning architecture (Sec. \ref{sec:benchmark_models}). Finally, in Sec. \ref{sec:transfer_benchmark}, we discuss different transfer models which we evaluate under Scenario 2. 

\subsection{Evaluation Scenarios and Dataset}
\label{sec:dataset}

We re-partition the dataset introduced by Ingber et al. \cite{ingber1998statistical} according to two experimental scenarios. Scenario 1 is used to benchmark our deep learning architecture against traditional classifiers. Scenario 2 is used to evaluate different transfer learning approaches using our deep learning architecture.

\begin{figure}[h]
	%\vspace{-.70cm}
\centering
\includegraphics[scale=.40]{Images/DataPartition.png}
\caption{\label{fig:partition} Middle row: Scenario 1 Benchmark Partition dataset split. Bottom row: Scenario 2 Transfer Learning dataset split}
% \caption{\label{fig:partition} Data partitions used for our original benchmarking (middle row) and transfer learning experiments (bottom row).  F1, F2, and F3 (up to \%75 of the remaining data) are sections of data used for fine tuning, leaving section T (25\%) for testing.}
\end{figure} 

%\subsubsection{Scenario 1: Performance Benchmarking}
\noindent
{\bf Scenario 1: Performance Benchmarking}
We stratify our train, test, and validation partitions according to subjects, i.e., each partition contains all trials form selected subjects and no subject overlap exists between partitions. Subjects were sampled without replacement according to a uniform random distribution. Of the subjects, 70\% were assigned to the train set, 20\% were assigned to the test set, and 10\% were assigned to the validation set, which was used to establish hyperparameters.


\noindent
{\bf Scenario 2: Transfer Learning Evaluation}
%\subsubsection{Scenario 2: Transfer Learning Evaluation}
In Scenario 2, we combine the training and validation partitions from Scenario 1 into one monolithic partition for pre-training transfer learning variants of our deep learning architecture. We then split our test partition from Scenario 1 into four novel equal-sized partitions: three fine-tuning partitions (F1,F2,F3) and a single test partition (T). Note that these splits were stratified over trials, sampled according to a uniform random distribution, meaning that F1, F2, F3, and T have subject overlap with respect to one another, but contain no subject overlap with respect to the pre-training partition.  



% Our subject data is split into typical partitions: 70\% training set, 20\% test set, and 10\% validation set. It is important to note here that our 70/20/10 splits were based on subjects, thus there were no overlapping subjects across the data sets.  Subjects used in training were not present in the validation set, nor in the test set.  This ensured that we were able to properly evaluate cross-subject performance among our classifiers.  For our initial experiments with traditional BCI classifiers, we held the validation set aside to validate model hyperparameters.  When training our baseline CNN for transfer learning experiments, we combined the training and validation sets into a single training set (using roughly 80\% of the subject trials), and we used an increasing sequence of proportions of the remaining 20\% from the transfer learning partition (i.e. the remaining 20\% of subjects) for three rounds of fine tuning (F1 through F3), leaving the remaining data (T) for validation.  Refer to Figure \ref{fig:partition} for data partition details.

% The sequence starts with using 25\% (F1) of the entire tuning partition (F1, F2, F3, and T), then 50\% (F1+F2), and finally 75\% (F1+F2+F3); T (the last 25\%) was consistently withheld for evaluation.  It should be clearly noted here that unlike the benchmark partition, the transfer learning partition (specifically T1, T2, and T3) did include overlapping subjects for fine tuning, but with \textit{no overlapping subject trials}. For both groups of experiments we segmented experiment trials by incrementing the training data and number of channels used in the baseline model.  We performed 216 experimental tests: 54 cross-task + 81 match/no-match + 81 high-risk/low-risk.  \textit{Note that due to the number of experiments, we show a selection of typical performance graphs under section \ref{sec:experiments}, offering subsequent graphs via supplemental content upon request}.


\begin{figure*}[!b]
        \centering
        \subfloat[High-Risk/Low-Risk]{\label{fig:alcoholicFull}
        \includegraphics[width=0.45\linewidth]{Images/roc_curves/alcoholic_detection_roc_60_100.png}}
        \hfill
        \subfloat[Match/Non-Match]{\label{fig:matchFull}
        \includegraphics[width=0.45\linewidth]{Images/roc_curves/match_detection_roc_60_100.png}}
    \caption{Scenario 1 benchmarks trained using all 60 channels per trial and 100\% of the trials in the training set.}
\end{figure*}

\subsection{Deep Learning Model Architecture}
\label{sec:dl_model}

We design our deep learning model to be amenable to learning from relatively few EEG trials in comparison to data volumes seen in other domains, e.g., computer vision, NLP, etc. To this end, we introduce a convolutional architecture which explicitly sums responses from feature maps of varying temporal bandwidth (i.e., parallel convolutions), rather than hierarchically stacking and pooling feature maps. The rationale here is to explicitly enforce consideration of salient data at multiple time scales, rather than rely on multi-time scale data propagating through stacked convolutions. While the latter design could be effective, we surmise that it is also more prone to overfitting on EEG-scale datasets. A number of changes/refinements could be integrated, e.g., channel-wise convolutions from \cite{lawhern2018eegnet}, which could be an interesting future study. We note that we do not conduct a thorough architectural exploration in this paper, since the aim of our present study is to explore cross-subject transfer learning rather than perform detailed architectural comparisons.

Specifically, our model takes as input pre-specified channels from one second of EEG data (one trial) at a sampling-rate of 256 Hz. This corresponds to 256 input dimensions per-channel. The input data is fed to three separate convolutional layers in parallel with varying kernel sizes of 3, 7, and 11, respectively. Each convolutional layer contains 32-filters and padding is performed so that outputs are equidimensional. The outputs are then summed element-wise to enforce explicit consideration of variable temporal bandwidths during optimization.  Max pooling is then applied, using a kernel size of 2, and the convolutional outputs are then rasterized to a 1D vector of 4096 dimensions. This vector is then passed through a layer normalization layer (LNorm), followed by an exponential linear unit (ELU) activation, then two subsequent stacks of linear layers followed by LNorm and ELUs reduce the dimension first to 1024 then to 128. A final linear layer squashes the output to 1D and a sigmoid link function is applied. 

% We use a simple CNN model constructed for our benchmark experiments as our baseline.  All of our models are trained on nothing more than the raw EEG data in the dataset.  The layers for the network are configured as follows:

% \begingroup
% \tiny%
% \begin{center}
% 	\fbox{\begin{minipage}{\linewidth}
			
% 			\textbf{Part I:}\\
% 			\-\ Conv1d(64, 32, kernel\_size=(3,), stride=(1,), padding=(1,))\\
% 			\-\ Conv1d(64, 32, kernel\_size=(7,), stride=(1,), padding=(3,))\\
% 			\-\ Conv1d(64, 32, kernel\_size=(11,), stride=(1,), padding=(5,))\\
% 			\-\ MaxPool1d(kernel\_size=2, stride=2, padding=0, dilation=1)\\
% 			\textbf{Part II:}\\
% 			\-\ Sequential\textbf{(}
% 			\-\ (0): LayerNorm((4096,), eps=1e-05)\\
% 			\-\ (1): ELU(alpha=1.0)\\
% 			\-\ (2): Dropout(p=0.5, inplace=False)\\
% 			\-\ (3): Linear(in\_features=4096, out\_features=1024, bias=True)\\
% 			\-\ (4): LayerNorm((1024,), eps=1e-05, elementwise\_affine=True)\\
% 			\-\ (5): ELU(alpha=1.0)\\
% 			\-\ (6): Linear(in\_features=1024, out\_features=128, bias=True)\\
% 			\-\ (7): LayerNorm((128,), eps=1e-05, elementwise\_affine=True)\\
% 			\-\ (8): ELU(alpha=1.0)\\
% 			\-\ (9): Linear(in\_features=128, out\_features=1, bias=True)\\
% 			\-\ (10): Sigmoid()\textbf{)}
			
% 	\end{minipage}}
% 	\captionof{Model}{The baseline CNN model used throughout our experiments.\label{fg:A}}
% \end{center}
% \endgroup

We trained the network for 7 epochs (the point at which repeated testing showed stabilized loss), using a minibatch size of 128 trials over approximately 3,700+ trials per epoch. For the baseline model, we utilized a cross-entropy loss between the model output and the corresponding (binary) label during backpropagation.



% The network was trained over 7 epochs (the point at which repeated testing showed stabilized loss), each containing a batch size of 128 trials over approximately 3,700+ trials. We use cross entropy loss during back propagation, which is the negative log-likelihood over the entire data set, presuming some probabilistic model on label noise: 
% \begin{equation}
% \label{eq:crossentropy}
% E_{\mbox{\tiny entropy}} = -\sum_{c_=1}^M y_o,_c\log(p_o,_c),
% \end{equation} 
% Here, $M$ is the number of possible classes and $p$ is the predicted probability that the observation $o$ is class $c$. In our case, we only need to distinguish between two classes: EP and not EP.  Presuming a \textit{Bernoulli} model on label noise, this is equivalent to the binary cross entropy loss function:\textit{binary cross entropy}:
% \begin{equation}
% \label{eq:binarycrossentropy}
% E_{\mbox{\tiny entropy}} = -(y\log(p)+(1-y)log(1-p))
% \end{equation}


\subsection{Benchmark Comparison Models (Scenario 1)}
\label{sec:benchmark_models}

To justify the application of our convolutional neural network (CNN) architecture, we benchmark raw performance against a number of more traditional classifiers in Sec. \ref{sec:experiments} on the Scenario 1 test partition. These classifiers include a dense feed-forward neural network (FFNN), logistic regression (LR), a random forest ensemble (RF), linear discriminant analysis (LDA), and Riemannian minimum distance to mean (RMDM). Where applicable, hyperparameters were selected using a grid search over the Scenario 1 validation set.
% Include FFNN architecture if space

\subsection{Transfer Learning Comparison Models (Scenario 2)}
 \label{sec:transfer_benchmark}
  For our transfer learning evaluation, we train several variations of our base CNN architecture (cf. \ref{sec:dl_model}) on the Scenario 2 training partition. We then fine-tune on the Scenario 2 fine-tuning partitions (F1, F1+F2, F1+F2+F3), and assess performance on the test partition. Model variations include:
  \begin{itemize}
  \item Fine-tuning with reduced learning rate with and without weight freezing on all but the penultimate layer. 
  \item Cross-task pre-training and fine-tuning. 
  \item Pre-training with an auto-encoder layer and mean squared error (MSE) reconstruction loss attached to the penultimate layer of the base representation.
  \item Pre-training a Siamese version of the base representation under a contrastive loss.
  \end{itemize}
 
 
 %Finally, we discuss the the dataset that we employ in our  experiments (Sec. \ref{sec:experiments}) and crucially, the splits that we use to assess transfer learning performance (Sec. \ref{sec:dataset}).

% This section describes… 
% Model we use (ref A)
% Comparison models against which we benchmark in results 
% -	Why we’re doing the benchmark – establish some viability of the DL model, i.e., do we need deep learning?
% Dataset for transfer learning experiments
% -	Splits and partitions
%\subsection {The Baseline (CNN) Model}
 
 %The second group of experiments focuses on deep transfer learning experiments.  Transfer learning falls under a more general category of machine learning referred to as \textit{representation learning}\cite{goodfellow2016deep}.  We experiment with adapting some of the deep learning-oriented tasks from recent studies for our own purposes; this approach allows us to quickly analyze and identify techniques that are the most performant. We evaluate results from a number of experiments: 
% \begin {itemize}
% \itemsep-0.2em
% \item Pre-train then fine-tune (w/ and w/o weight-freezing; same task)
% \item Pre-train then fine-tune (cross-task)
% \item Pre-train w/ auto-encoder then fine-tune
% \item Pre-train w/ Siamese loss then fine-tune
% %\item Pre-train w/ multi-task loss then fine-tune
% \end {itemize} 

% Pre-training consists of the initial training of our base CNN model and all of its layers.  Fine-tuning is where the transfer learning happens.  For the base model, this entails either freezing weights in the convolutional layers or not.  The sections that follow elaborate on each experiment listed above. 





% An ideal BCI classifier would offer a high degree of scalability across large quantities of heterogeneous EEG data while requiring relatively little data and time to customize for any particular application. While this idealized classifier may not be fully realized, we explore how closely we might get to achieving such a model through 2 experiment groups: (1) experiments around traditional BCI classifiers and (2) experiments that unpack deep transfer learning and fine-tuning.





% An ideal BCI classifier would offer a high degree of scalability across large quantities of heterogeneous EEG data while requiring relatively little data and time to customize for any particular application. While this idealized classifier may not be fully realized, we explore how closely we might get to achieving such a model through 2 experiment groups: (1) experiments around traditional BCI classifiers and (2) experiments that unpack deep transfer learning and fine-tuning.

% %The ideal BCI classifier offers a high degree of scalability across large quantities of heterogeneous electroencephalographic data while requiring relatively little data and time to customize for any particular application. We explore how closely we might approach this idealistic model through 2 experiment groups: (1) experiments around traditional BCI classifiers and (2) experiments that unpack deep transfer learning and fine-tuning.

% The first group consists of experiments that pit a convolutional neural network (CNN) against a dense feed-forward neural network (FFNN) vs. logistic regression (LR) vs. random forest (RF) vs. linear discriminant analysis (LDA) vs. Riemannian minimum distance to mean (RMDM).  The second group of experiments focuses on deep transfer learning experiments.  Transfer learning falls under a more general category of machine learning referred to as \textit{representation learning}\cite{goodfellow2016deep}.  We experiment with adapting some of the deep learning-oriented tasks from recent studies for our own purposes; this approach allows us to quickly analyze and identify techniques that are the most performant. We evaluate results from a number of experiments: 
% \begin {itemize}
% \itemsep-0.2em
% \item Pre-train then fine-tune (w/ and w/o weight-freezing; same task)
% \item Pre-train then fine-tune (cross-task)
% \item Pre-train w/ auto-encoder then fine-tune
% \item Pre-train w/ Siamese loss then fine-tune
% %\item Pre-train w/ multi-task loss then fine-tune
% \end {itemize} 

% Pre-training consists of the initial training of our base CNN model and all of its layers.  Fine-tuning is where the transfer learning happens.  For the base model, this entails either freezing weights in the convolutional layers or not.  The sections that follow elaborate on each experiment listed above. 


% %\subsection{The Dataset}
% \subsection{Dataset Overview and Partitions}
% \label{sec:dataset}

% In order to study cross-subject transfer using classifiers which do not require engineered features, we require a dataset with sufficient subjects and samples to fit our proposed experimental models. As one of these is a deep learning model, this means that we need several thousand samples, ideally with samples distributed uniformly over subject trials.  %TODO: citation on the several thousand 
% We utilize a well-curated dataset from a large study that examined EEG correlates of genetic predisposition to alcoholism \cite{ingber1998statistical}. While the dataset is somewhat dated, it is one of the few publicly available EEG datasets that has the aforementioned characteristics that we require for this study.


% %We discovered a well-curated dataset from a large study that examined EEG correlates of genetic predisposition to alcoholism (1995). While the dataset is somewhat dated, it is one of the few publicly available EEG datasets of sufficient size and labeling that meets our needs for this study.  Several papers can be found that have used and/or describe the dataset chosen for this research: \cite{ingber1982statistical, shobeihi2006classification, bajwa2016neurokey, ccokyilmaz2011classification, lopes2004classification} 

% Our subject data is split into typical partitions: 70\% training set, 20\% test set, and 10\% validation set. It is important to note here that our 70/20/10 splits were based on subjects, thus there were no overlapping subjects across the data sets.  Subjects used in training were not present in the validation set, nor in the test set.  This ensured that we were able to properly evaluate cross-subject performance among our classifiers.  For our initial experiments with traditional BCI classifiers, we held the validation set aside to validate model hyperparameters.  When training our baseline CNN for transfer learning experiments, we combined the training and validation sets into a single training set (using roughly 80\% of the subject trials), and we used an increasing sequence of proportions of the remaining 20\% from the transfer learning partition (i.e. the remaining 20\% of subjects) for three rounds of fine tuning (F1 through F3), leaving the remaining data (T) for validation.  Refer to Figure \ref{fig:partition} for data partition details.

% The sequence starts with using 25\% (F1) of the entire tuning partition (F1, F2, F3, and T), then 50\% (F1+F2), and finally 75\% (F1+F2+F3); T (the last 25\%) was consistently withheld for evaluation.  It should be clearly noted here that unlike the benchmark partition, the transfer learning partition (specifically T1, T2, and T3) did include overlapping subjects for fine tuning, but with \textit{no overlapping subject trials}. For both groups of experiments we segmented experiment trials by incrementing the training data and number of channels used in the baseline model.  We performed 216 experimental tests: 54 cross-task + 81 match/no-match + 81 high-risk/low-risk.  \textit{Note that due to the number of experiments, we show a selection of typical performance graphs under section \ref{sec:experiments}, offering subsequent graphs via supplemental content upon request}.

% \begin{figure}[h]
% 	%\vspace{-.70cm}
% \centering
% \includegraphics[scale=.40]{Images/DataPartition.png}
% \caption{\label{fig:partition} Data partitions used for our original benchmarking (middle row) and transfer learning experiments (bottom row).  F1, F2, and F3 (up to \%75 of the remaining data) are sections of data used for fine tuning, leaving section T (25\%) for testing.}
% \end{figure} 





==> sections/Conclusion.tex <==
\section{Conclusions}
\label{sec:conclusion}
Transfer learning can substantially augment performance and reduce training data requirements for BCI.  Comparing our baseline performance in Figure \ref{fig:transferMatchRocs} with our binary transfer results in Figure \ref{fig:transferMatchBinaryNoFreezeRocs} shows that even when using 1/3 of the transfer dataset to pre-train, our model substantially outperforms the baseline trained on the full transfer set by nearly 10\% in terms of area under the ROC curve. For the HR/LR results there are performance gains across all training sizes.

 The most prominent evidence brought to light here is that there is no single classifier in the group that performs well across tasks.  For short latent EP, our fine-tuned binary CNN model outperforms every other method we explored in this work, including our selected traditional BCI classifiers.  For long, sustained ERP patterns our Siamese approach outperformed all others by a large margin.  The performance trend continues upward as we increase the amount of data used for both training and fine-tuning, until we run out of data.



==> sections/Discussion.tex <==
\section{Discussion}
\label{sec:discussion}

To better understand \textit{what} our models are learning we explored how to exploit interpretable explainers in novel ways.  Specifically, can we know how our models conjure their predictions, and can we determine whether or not those outputs are learning on features we would expect \cite{ribeiro2016should,doshi2017towards,molnar2019interpretable}?  Since there isn't a one-size-fits-all method towards \textit{interpretability}, we present evidence for our chosen approach for BCI EEG interpretability: integrated gradients (IG).    

Unlike metrics commonly used to analyze performance (accuracy, sensitivity, specificity and efficiency), the safety and trustworthiness of our models are rarely precisely quantified; however, these seemingly ancillary objectives may become very important in a given application and setting \cite{vellido2019importance,tjoa2019survey,lahav2018interpretable}.  For example, BCI holds much potential for use as a tool in clinical settings.  Such applications may aid clinicians and patients in the diagnosis and treatment of addiction disorders, learning disabilities, depression, dementia, epilepsy and more \cite{minguillon2017mobile, nakanishi2017detecting, al2017review,chatelle2018feasibility,pan2020prognosis,belkacem2020brain,ctarcuaapplication,roy2019deep}.  Under these circumstances, we must ensure the highest trust and reliability in our models.   

The authors of \cite {lundberg2017unified} provided evidence that many popular local interpretability methods, including the IG, Interpretable Model-Agnostic Explanations (LIME), and SHapley Additive exPlanations (SHAP) employ (essentially) the same explanation method: \textit{the additive feature attribution} (AFA) method.  AFA has three main properties which we review, local accuracy, missingness, and consistency.

Let \(f\) be the (complex) model we will interpret and \(g\) be the explainer model. \(f(x)\) is a prediction based on a single sample input \(x\).  Our explainers accept simplified input \(x'\) that map to the original input through the mapping function \(x=h_x\).  Local methods will (reasonably) ensure that \(g(z')\approx f(h_x (z'))\) whenever \(z'\approx x'\).  Keep in mind that because \(h_x\) is specific to the current input \(x\), \(h_x(x')=x\), despite \(x'\) containing less information than \(x\).

\begin{equation}
	\label{eq:additive_feature_attrib}
	\textrm{let }
	g(z') = \phi_0+\sum_{i_=1}^n \phi_i z'_i, 
\end{equation} 
where \(z'\in\{0,1\}^n\), \(n\) is the number of simplified input features, and \(\phi_i \in R\).
%\captionof{figure}{Additive feature attrribution methods have an explaination model that is a linear function of binary variables \cite {lundberg2017unified}}
These models all attribute an effect \(\phi_i\) to every feature, and summing these effects approximates the output of the original model prediction \(f(x)\). In short, the AFA method is simply a linear regression over a binary mask where deviations are guaranteed to be linear for local instances (think \textit{locality}).  This is also referred to as \textit{local accuracy}.  

\begin{equation}
	\label{eq:local_accuracy}
	f(x)=g(x') = \phi_0+\sum_{i_=1}^n \phi_i x'_i, 
\end{equation} 

In addition to this property, AFA method highlights two more ideal properties present in good interpretability models: property 2 is referred to as \textit{missingness}; it constrains certain features to have no attributed impact where 
\(x'\)=0.  
\begin{equation}
	\label{eq:additive_feature_prop2}
	x'=0 \Longrightarrow \phi_i = 0 
\end{equation} Property 3 is \textit{consistency}; the idea behind it states that an input's attribution should not decrease if a model changes so that some simplified input's contribution increases or stays the same regardless of other inputs, that input's attribution should not decrease \cite{lundberg2017unified,molnar2019interpretable}.

Let \(f(z')\)=\(f(h_x (z'))\) and \(z \backslash j'\) indicate that \(z'_j=0\) for any two models \(f and f'\) that satisfy:
\begin{equation}
	\label{eq:additive_feature_prop3}
	f'_x(z') - f'_x(z'_{\backslash j})\geq f_x(z') - f_x(z'_{\backslash j})
\end{equation}

for all input \(z' \in \{0,1\}^M\), then:
\(
\phi_j(f',x)\geq \phi_j(f,x)
\)

\subsection {Integrated Gradients (IG)}\label{section:IG}
%% intro to method, how applied here
In this seminal paper \cite{sundararajan2017axiomatic} the authors introduce IG as a self-evident (\textit{axiomatic}) method towards explainability; additive feature attribution (i.e. \textit{completeness}) can be viewed thusly: 
\textbf{\(\sum_{i_=1}^n IntegratedGrads_i(x) = F(x) - F(x')\)}, where \(x\) is the original input, \(x'\) is the baseline, and \(F: R^n\rightarrow [0,1]\) is the output of a neural network, assuming \(F : R^n\rightarrow R\) is \textit{differentiable almost everywhere}.

Formally, the integrated gradients defines the contribution of a given attribute, \(i\) for an input \(x\) and baseline \(x'\) thusly: let \(\frac{\partial F(x)}{\partial x_i}\) be the gradient of \(F(x)\) along the \(ith\) dimension. 
\begin{equation} \label{eq:IG}
	\begin{split}
		IntegratedGrads_i(x)::=\\ 
		(x_i-x'_i) \times \int_{\alpha=0}^1 \frac{\partial F(x'+\alpha \times (x-x'))}{\partial x_i}
	\end{split}
\end{equation}

Put another way, integrated gradients will aggregate the gradients along the inputs that fall on the (straight) line between the baseline and the input\cite{sundararajan2017axiomatic}.  This idea shows that IG is among a group of methods known as \textit{path methods}. Unlike many gradients methods used to interpret neural networks, IG avoids \textit{saturation} by integrating over a \textit{path}, which tells us, when scaled along this path, which attribute increased the output towards the correct classification\cite{sturmfels2020visualizing,sundararajan2017axiomatic}. 

\subsection{An Approach to Explainability}
 For our purposes we approach explainers as being a part of a decision support system (DSS) that may assist both technical and nontechnical persons assessing the performance of complex learning models by producing interpretable models that are much easier for humans to examine and assess.  We place the human in the loop so that we may learn the regions within the EEG signals where each classifier placed the greatest importance (highest weights).  Knowing this information may allow us to gain a better understanding of our data as well as our classifier models.  To our knowledge this work is the first to apply integrated gradients explainers to electroencephalography and BCI.  For a given model and threshold, we performed the following on the top performers for match/no-match and high-risk/low-risk:

\begin {enumerate}
\itemsep-0.25em
\item We start with the predictions (scores) related to the pretrained model.
\item For each examined sample (positive or negative) label, create an explainer:
\begin {enumerate}
\itemsep-0.25em
\item Evaluate the model using an allotment of test data.
\item Collect and rank all TP and TN scores using a chosen prediction threshold.
\item Aggregate the data samples across channels for the top N scores for each TP and TN
\item Obtain the feature attributions (i.e. weights) via integrated gradients (this results in a 2D array of IG weights for each channel and sample therein).
\item Using these weights, create a temporal \& spatial heat map that corresponds to each channel and its attributed factor.
\item Similarly, we use these weights to create a temporal and spatial dipole heat map that depicts the spatial and temporal contribution of each feature in the sample.
\end {enumerate}
\item We now have a way of examining what a classifier learns; we can better visualize from different perspectives what our models are learning.
\item We can examine each explainer to get an idea of which channels contribute positively or negatively to the overall prediction.
\end {enumerate}

\subsection{Interpreting the Explainers}

It is important that the reader does not discount the fact that examining information related to EEG \textit{requires} a certain level of knowledge in neuroscience, electroencephalography, BCI, or some combination of these topics.  Interpretability and related explainers are tools we seek to provide so that subject matter experts may evaluate what our models are learning.  We provide an interpretation of the explainers below so that readers without any background may examine what these explainers show.

In EP (match/no-match) we would expect the presence of early latent activity in EEG between 0 and 400 milliseconds after the stimulus is introduced to the subject; therefore, we should see some indication that our classifiers have learned some sort of representation of this early temporal activity.  Similarly, for sustained ERP (high-risk vs low-risk), we might see some sort of difference in how regions of the brain react to stimulus over time between high-risk and low-risk subjects.  According to our data analysis, normal progression should start towards the temporal region of the brain and eventually progress towards the frontal lobes.  We expect our models to have learned these differences in spatial progression between high-risk and low-risk subjects.  We fashioned our explainers to convey these details, assuming that they exist.

We created 3 types of visuals around our explainers: (1) A spatial dipole heat map representing weighted features as they relate to regions of the brain over an entire 1-second of time; represents spatial details only, (2) a joint temporal dipole heat map that represents weighted features as they progress over the length of a trial; also shows weights spatially and temporally for each channel, and (3) a channel heat map that shows how each feature's weighted contributions change over time within each channel.  We show several examples of these explainers and how we interpreted them.  Keep in mind that these images depict feature contributions (i.e. weighted features) towards a particular classification; they do not necessarily directly correspond to actual EEG amplitude.


\subsubsection{High Risk Vs. Low Risk Explainers}
Choosing a threshold of .51 we took all true positives (representing high-risk) and all true negatives (representing low-risk) and created explainers for each category.  Figures \ref{fig:tp_alcoholic_avg_all_dipole} and \ref{fig:SiameseAlcoholic_TP_ALL_joint_IG} depict the same things in different ways: all depict how EEG features contributed to high-risk classification.  Figures \ref{fig:tp_nonalcoholic_avg_all_dipole} and \ref{fig:SiameseAlcoholic_TN_ALL_joint_IG} all depict how EEG features contributed to low-risk classification.  

Comparing aggregated dipoles across subjects in Figures \ref{fig:tp_alcoholic_avg_all_dipole} and \ref{fig:tp_nonalcoholic_avg_all_dipole} provides us with the spatial differences between the two groups.  We can clearly see these differences when the images are juxtaposed.  These images tell us nothing about what was learned of ERP progression over time, but could be useful if we're not concerned with knowing those temporal details; this would depend on the application.

To gain a better understanding about what our Siamese transfer models learned about temporal progression, we can compare Figures \ref{fig:SiameseAlcoholic_TP_ALL_joint_IG} and \ref{fig:SiameseAlcoholic_TN_ALL_joint_IG}.  The biggest differences in the way the features contribute over time seem to be between the frontal lobes and the temporal lobe.  Low-risk subjects have large oscillatory feature swings starting in the temporal lobe that contribute to most of the activity within the first half of a trial, then shifting to the frontal lobes while high-risk subjects seem to show features related to the frontal lobes contributing more throughout the entire trial.  Interestingly enough, the low-risk group (also the control group) shows patterns that seem to jibe with what we'd expect to see in a normal subject.  High-risk is clearly different in this regard. 

If we change the temporal perspective slightly, we get yet another piece of information not readily visible in the first two representation.  Figures \ref{fig:SiameseAlcoholic_TP_ALL_joint_IG_heat} and \ref{fig:SiameseAlcoholic_TN_ALL_joint_IG_heat} depict temporal heat maps.  At first glance, these maps seem to introduce nothing but confusion; however, looking more closely at these two maps shows that is less “noise” in the low-risk map.  This could indicate that certain low-risk ERP features are more pronounced, overwhelming other less relevant features, leaving those features with barely any contribution (i.e. neutral weight).  This could be an indicator that some users of certain BCI systems may require systems that are better trained on more data from their respective clinically designated risk groups. 
%====== ERP Siamese Model Visuals ============

\begin{figure}[h]
	\centering
	\includegraphics[scale=.60]{Images/explainers/SiameseAlcoholic_TP_ALL_joint_IG_dipole_IG.png}
	\caption{\label{fig:tp_alcoholic_avg_all_dipole} A dipole heat map representing what our Siamese network learned over all high-risk tasks.  This image shows aggregated feature contributions (depicted through IG) across all TP high risk (alcoholic) subjects averaged across the entire length of a 1-second trial, showing which channels spatially contributed negatively (blue) or positively (red) towards the prediction.}
\end{figure}

\begin{figure}[h]
	\centering
	\includegraphics[scale=.27]{Images/explainers/SiameseAlcoholic_TP_ALL_joint_IG.png}
	\caption{\label{fig:SiameseAlcoholic_TP_ALL_joint_IG} A joint temporal dipole heat map representing what our Siamese network learned over all high-risk tasks.  This image shows aggregated feature contributions (depicted through IG) across all TP high risk (alcoholic) subjects through time over the entire length of a 1-second trial, showing which channels spatially and temporally contributed negatively (blue) or positively (red) towards the prediction.  Below the dipole maps we are able to follow the contributions of each EEG channel through time.}
\end{figure}

\begin{figure}[h]
	\centering
	\includegraphics[scale=.60]{Images/explainers/SiameseAlcoholic_TN_ALL_joint_IG_dipole_IG.png}
	\caption{\label{fig:tp_nonalcoholic_avg_all_dipole} A dipole heat map representing what our Siamese network learned over all \textbf{low-risk} tasks.  This image shows aggregated feature contributions (depicted through IG) across all low risk (non-alcoholic) subjects averaged across the entire length of a 1-second trial, showing which channels spatially contributed negatively (blue) or positively (red) towards the prediction.}
\end{figure}

\begin{figure}[h]
	\centering
	\includegraphics[scale=.25]{Images/explainers/SiameseAlcoholic_TN_ALL_joint_IG.png}
	\caption{\label{fig:SiameseAlcoholic_TN_ALL_joint_IG} A joint temporal dipole heat map representing what our Siamese network learned over all low-risk tasks.  This image shows aggregated feature contributions (depicted through IG) across all low risk (non-alcoholic) subjects through time over the entire length of a 1-second trial, showing which channels spatially and temporally contributed negatively (blue) or positively (red) towards the prediction.  Below the dipole maps we are able to follow the contributions of each EEG channel through time.}
\end{figure}

\begin{figure}[h]
	\centering
	\includegraphics[scale=.19]{Images/explainers/SiameseAlcoholic_TN_ALL_joint_IG_heat.png}
	\caption{\label{fig:SiameseAlcoholic_TN_ALL_joint_IG_heat} A temporal heat map representing what our Siamese network learned over all low-risk tasks.  This image shows aggregated feature contributions (depicted through IG) across all low risk (non-alcoholic) subjects through time over the entire length of a 1-second trial, showing which channels contributed negatively or positively towards the prediction.}
\end{figure}

\begin{figure}[h]
	\centering
	\includegraphics[scale=.19]{Images/explainers/SiameseAlcoholic_TP_ALL_joint_IG_heat.png}
	\caption{\label{fig:SiameseAlcoholic_TP_ALL_joint_IG_heat} A temporal heat map representing what our Siamese network learned over all high-risk tasks.  This image shows aggregated feature contributions (depicted through IG) across all TP high risk (alcoholic) subjects through time over the entire length of a 1-second trial, showing which channels contributed negatively or positively towards the prediction.}
\end{figure}

\subsection{Match Vs. No-Match Explainers}
Just as we did with the high-risk vs low-risk explainers for our Siamese model, we wish to gain some understanding into what our binary transfer model is learning about match/no-match trials.  Choosing a threshold of .51 we took all true positives (representing match) and all true negatives (representing no-match) and created explainers for each category. Unlike high-risk vs. low-risk, we expect to see most activity (i.e. most contributions) somewhere in the vicinity between 0 and 400 milliseconds.  Comparing the aggregate dipoles across subjects in Figures \ref{fig:BinaryMatch_TP_ALL_joint_IG_dipole} and \ref{fig:BinaryMatch_TN_ALL_joint_IG_dipole} provides us with the spatial differences between the two trials; however, we are much more interested in knowing if our model has learned the difference between P3a and P3b.

Contrasting Figures \ref{fig:BinaryMatch_TP_ALL_joint_IG} and \ref{fig:BinaryMatch_TN_ALL_joint_IG} we can clearly see that there is \textit{similar} progression of feature contributions in the temporal region between 0 and 400 milliseconds - just as we would expect from a classifier that was properly learning on early to mid latent EP features.  Notices how most features after 400 milliseconds have barely any positive contributions.  Our classifier is clearly learning the proper temporal aspects.   If we examine the differences in these contributions between match and no-match, we can see the differences made clearer there, too.  

The temporal heat maps in Figures \ref{fig:BinaryMatch_TP_ALL_IG_heat} and \ref{fig:BinaryMatch_TN_ALL_IG_heat} provide a better picture of which features in each channel contribute the most in the early temporal regions. We could us these sorts of heat maps to determine which channels we may omit to create less expensive, more portable BCI systems by cutting out channels that contribute less to the overall prediction coming from our classifiers. 

%====== EP Binary Model Visuals ============
\begin{figure}[h]
	\centering
	\includegraphics[scale=.19]{Images/explainers/BinaryMatch_TP_ALL_IG_heat.png}
	\caption{\label{fig:BinaryMatch_TP_ALL_IG_heat} A temporal heat map representing what our binary (CNN) network learned over all \textbf{match} tasks.  This image shows aggregated feature contributions (depicted through IG) across all TP match tasks through time over the entire length of a 1-second trial, showing which channels contributed negatively or positively towards the prediction.}
\end{figure}

\begin{figure}[h]
	\centering
	\includegraphics[scale=.19]{Images/explainers/BinaryMatch_TN_ALL_IG_heat.png}
	\caption{\label{fig:BinaryMatch_TN_ALL_IG_heat} A temporal heat map representing what our binary (CNN) network learned over all \textbf{no-match} tasks.  This image shows aggregated feature contributions (depicted through IG) across all TN match tasks through time over the entire length of a 1-second trial, showing which channels contributed negatively or positively towards the prediction.}
\end{figure}

\begin{figure}[h]
	\centering
	\includegraphics[scale=.60]{Images/explainers/BinaryMatch_TP_ALL_joint_IG_dipole.png}
	\caption{\label{fig:BinaryMatch_TP_ALL_joint_IG_dipole} A dipole heat map representing what our binary (CNN) network learned over all \textbf{match} tasks.  This image shows aggregated feature contributions (depicted through IG) across all TP match tasks averaged across the entire length of a 1-second trial, showing which channels spatially contributed negatively (blue) or positively (red) towards the prediction.}
\end{figure}

\begin{figure}[h]
	\centering
	\includegraphics[scale=.28]{Images/explainers/BinaryMatch_TP_ALL_joint_IG.png}
	\caption{\label{fig:BinaryMatch_TP_ALL_joint_IG} A joint temporal dipole heat map representing what our binary (CNN) network learned over all \textbf{match} tasks.  This image shows aggregated feature contributions (depicted through IG) across all TP match task through time over the entire length of a 1-second trial, showing which channels spatially and temporally contributed negatively (blue) or positively (red) towards the prediction.  Below the dipole maps we are able to follow the contributions of each EEG channel through time.}
\end{figure}

\begin{figure}[h]
	\centering
	\includegraphics[scale=.60]{Images/explainers/BinaryMatch_TN_ALL_joint_IG_dipole.png}
	\caption{\label{fig:BinaryMatch_TN_ALL_joint_IG_dipole} A dipole heat map representing what our binary (CNN) network learned over all \textbf{no-match} tasks.  This image shows aggregated feature contributions (depicted through IG) across all TN match tasks averaged across the entire length of a 1-second trial, showing which channels spatially contributed negatively (blue) or positively (red) towards the prediction.}
\end{figure}

\begin{figure}[h]
	\centering
	\includegraphics[scale=.25]{Images/explainers/BinaryMatch_TN_ALL_joint_IG.png}
	\caption{\label{fig:BinaryMatch_TN_ALL_joint_IG} A joint temporal dipole heat map representing what our binary (CNN) network learned over all \textbf{no-match} tasks.  This image shows aggregated feature contributions (depicted through IG) across all TN match task through time over the entire length of a 1-second trial, showing which channels spatially and temporally contributed negatively (blue) or positively (red) towards the prediction.  Below the dipole maps we are able to follow the contributions of each EEG channel through time.}
\end{figure}

==> sections/Experiments-Old.tex <==
\section{Experiments}
\label{sec:experiments}

The data includes 122 subjects with 2 groups: alcoholic predisposition (77 people) and control group (45 people). It is a balanced dataset in that trials were split roughly 50-50 between a form of popular go/no-go experiments often used in biological research with animal and human subjects (explained later as match/no-match trials). 64 scalp electrodes (channels) were used with a standard 10/20 extended spatial configuration. There were 120 trials per subject where recordings were segmented into 1-second windows which included 3.9ms epochs.  To elicit event-related potentials (ERPs), a delayed matching-to-sample task was used. Two images appeared in succession with a 1.6 second inter-stimulus interval. First, a random image (S1) from the set was displayed to the subject for 300ms. The image that followed was either a match to the first (S2 Match), or a different image altogether (S2 No Match).  All trials were randomized and balanced; one half of the trials contained matches, while the other half did not. 

\subsection{Model Benchmark Experiments}
 Classifiers were trained to detect two different pieces of information from the EEG dataset: (1) whether a given subject was part of the high-risk (HR) alcoholic group or the low-risk (LR) control group, and (2) whether a given subject trial resulted in a match or no-match scenario (labeled as 1 = match, 0 = no-match).

 We measured several aspects related to performance for each classifier: (1) which task a given classifier performed best at: (a) short elicited response patterns (match vs no-match) or (b) sustained ERP patterns (as in clinic classification or motor imagery), (2) which classifiers performed well with increased channels (which may increase both signal and noise), and (3) which classifiers performed well with less training data.

 We performed in total 126 experiments under 2 task groups: (1) match vs no-match and (2) high-risk (HR) vs low-risk (LR). There were 9 experiments performed for each of the 7 classifiers for each task group.  For each group we performed 3 sets of tests where each set used an increasing amount of the allocated training data (i.e. increased amount of trials for each subject).  Within each test we incrementally increased the number of channels used during the training process.  
 
 The tests progressed as follows: (1) Each test in each experiment started out using 10\% of the trials for each subject of the original 70\% training set, then the training set was incremented to 50\% of the trials, and finally 100\% of the subjects' trials. (2) Within each test, we started the test with 8 channels, then 12 channels, and finally 60 channels.  Selected channels correspond to typical BCI configurations.  (3) Performance for each classifier was recorded, ROC curves were compared relative to all other classifiers withing each experiment.  (4) Thresholds were evaluated to determine how well each classifier would perform under a given context (critical vs non-critical).

\subsection{Receiver Operating Characteristic (ROC) Curves}

We examine receiver operating characteristic (ROC) curves related to our experimental results for both the shape of the curves as well as the area under the curves (AUC).  To see additional ROC curves resulting from these experiments, please request our \textit{supplemental material}.
\begin{figure}
	\begin{tabular}{cc}
		%\includegraphics[width=46mm]{Images/roc_curves/match_detection_roc_8_10.png} &  \hspace{-1.1cm} 
		%\includegraphics[width=40mm]{Images/roc_curves/match_detection_roc_12_10.png}&  %\hspace{-1.1cm}\\
		%\hspace{-.90cm}
		%\includegraphics[width=40mm]{Images/roc_curves/match_detection_roc_60_10.png} \\
		%\includegraphics[width=46mm]{Images/roc_curves/match_detection_roc_8_50.png} &  \hspace{-1.1cm}
		 %\includegraphics[width=50mm]{Images/roc_curves/match_detection_roc_12_50.png} \hspace{-.90cm}
		%\includegraphics[width=50mm]{Images/roc_curves/match_detection_roc_60_50.png} \\
		%\includegraphics[width=46mm]{Images/roc_curves/match_detection_roc_8_100.png} &  \hspace{-1.1cm}
		\includegraphics[width=40mm]{Images/roc_curves/match_detection_roc_12_100.png}& %\hspace{-.90cm}
		\hspace{-.90cm}
		\includegraphics[width=40mm]{Images/roc_curves/match_detection_roc_60_100.png}\\ 
	\end{tabular}
\caption{\label{fig:matchRocs}ROC curves and AUC for match/no-match experimentation.  These curves show performance with 12 and 60 channels using 100\% of the available training data.}
\end{figure}

\begin{figure}
	\begin{tabular}{cc}
		%\includegraphics[width=46mm]{Images/roc_curves/alcoholic_detection_roc_8_10.png} &  \hspace{-1.1cm}
		\includegraphics[width=40mm]{Images/roc_curves/alcoholic_detection_roc_12_10.png}& % \hspace{-1.1cm}
		\hspace{-.90cm}
		\includegraphics[width=40mm]{Images/roc_curves/alcoholic_detection_roc_60_10.png}\\ 
		%\includegraphics[width=46mm]{Images/roc_curves/alcoholic_detection_roc_8_50.png} &\hspace{-1.1cm}
		 %\includegraphics[width=50mm]{Images/roc_curves/alcoholic_detection_roc_12_50.png} \hspace{-.90cm}
		%\includegraphics[width=50mm]{Images/roc_curves/alcoholic_detection_roc_60_50.png}\\
		%\includegraphics[width=46mm]{Images/roc_curves/alcoholic_detection_roc_8_100.png} &  \hspace{-1.1cm}
		\includegraphics[width=40mm]{Images/roc_curves/alcoholic_detection_roc_12_100.png} & %\hspace{-.90cm}
		\hspace{-.90cm}
		\includegraphics[width=40mm]{Images/roc_curves/alcoholic_detection_roc_60_100.png}\\ 
	\end{tabular}
\caption{\label{fig:alcoholichRocs}ROC curves and AUC for high-risk/low-risk experimentation.  The top row shows performance with 12 and 60 channels using only 10\% of the available training data.  The bottom row shows performance with 12 and 60 channels using 100\% of the available training data.}
\end{figure}

\subsection{Match Vs No-match Experiments}

This task group allowed us to experiment with how well our classifiers might perform in BCI designed for actionable EP.  These types of systems users to communicate with others, browse the internet, adjust environmental controls, flip lights on of off, etc..  Typically, they are built around visually evoked potentials or other early to mid-level latent responses such as P300.

 There are a few interesting things to note about our classifiers in in Figure \ref{fig:matchRocs}.  The Riemannian (RMDM) model did not perform at all for these sorts of tasks, performing no better than random chance; this was true for any test, regardless of the number of channels or the amount of training data.  Clearly, the RMDM classifier does not perform well as-is against raw EEG data where detecting short EP patterns is a requirement.  One paper saw similar results on this type of EP (P300), but surmised it was due to applying a prior spatial filter to the data \cite{congedo2019riemannian}.  The authors' conclusion is likely inaccurate, since our data has no such filter applied to it. 

When the amount of training data was low, LDA showed an interesting trend of increasingly better performance as the number of channels (i.e. feature space) increased.  LDA outperformed all other classifiers but gradient boosting (GB) when all 60 channels were used with the lowest amount of training data (see \ref{fig:matchRocs}).  LDA contends well with small amounts of high dimensional data; however, as the amount of data increases other more robust classifiers catch up and then surpass the performance of LDA.  This suggests that LDA does not generalize well across subjects and it doesn't contend well with increasing noise.  This suggests that LDA would require re-training for any user over a short period of time, since EEG for any subject is non-stationary over time.

Unlike LDA, the logistic regression (LR) model scaled better as the amount of training data was increased, showing good stability with 8 and 12 channels, but performance drops considerably with 60 channels.  This suggests that LR cannot scale well with high dimensional feature space, but generalizes across subjects where LDA cannot.  Examine the bottom row in Figure \ref{fig:matchRocs}.

Both of our ensemble methods, random forest (RF) and gradient boosting (GB) showed stable performance across all the tests.  Boosting shows a consistent edge in performance over random forest as well as a bit more stability, albeit a slight edge in both cases.  In fact, GB was outperformed only by our convolutional neural network (CNN) model when the full test set and all channels were in play; nevertheless, GB proved stable across all test. This suggests that ensemble approaches remain powerful, relevant models to BCI systems.  

Both feed-forward neural network (FFNN) and the convolutional neural network (CNN) were the overall top performers.  Overall, the CNN model outperforms our FFNN as the data and number of channels increases.  The FFNN shows some potential to perform slightly better on smaller quantities with a lesser feature space, showing that deep learning models have potential for good performance and generalization across subjects, noise (i.e. variance) and feature space across both temporal and spatial dimensions.  

\subsection{High-Risk Vs Low-Risk Experiment}
This series of tests evaluates how well our models might perform for BCI systems meant for clinical diagnostics or motor imagery.  These types of ERPs carry sustained patterns across longer periods of time, and are usually consistently cyclical in nature.  These ERPs can help clinicians identify pathological patterns in a subjects brain, or allow a user to move a prosthetic arm, hand, leg or wheelchair. Initially, we had expected results similar to the math/no-match experiment.  We refer you to Figure \ref{fig:alcoholichRocs}.

The RMDM model was the top performer in these tests among traditional classifiers.  While it's clear the RMDM (as-is) cannot contend with the shorter, noisier EP related tasks performed in the previous set of experiments, it shows here that RMDM does have an ability to draw out other patterns from ERP that none of the other classifiers could learn with these experiments.  RMDM remained stable and performs well regardless of how much training data was used.  In fact, performance increased when we stepped up from 8 channels to 12.  However, there are limits; RMDM quickly deteriorated, becoming less stable when incorporating all channels.  This demonstrates that there is clearly a limit to the dimensions in a given feature space.  This paper seems to back up this assumption: \cite{rodrigues2019exploring}.  The other classifiers performed poorly here, and showed a fair amount of instability.  

\subsection {Transfer Learning Experiments}

Given a source domain \(D_S\) and a (learning) task \(T_S\), a target domain \(D_T\) and its task \(T_T\), transfer learning seeks to improve the learning of the predictive target function \(f_T(\cdot)\) in \(D_T\) by using \textit{knowledge} in \(D_S\) and \(T_S\), assuming $(D_S \ne D_T), or (T_S \ne T_T)$.  For purposes of this study, a domain \(D\) is a \textit{subject} or number of subjects whose EEG data is used to train a specific model, and a task \(T\) is mapped to EP or ERP we wish to associate with actions related to context with a specific BCI.  

Here, evaluate results from a number of experiments: 
\begin {itemize}
\itemsep-.25em
\item Pre-train then fine-tune (w/ and w/o weight-freezing; same task)
\item Pre-train then fine-tune (cross-task)
\item Pre-train w/ auto-encoder then fine-tune
\item Pre-train w/ Siamese loss then fine-tune
%\item Pre-train w/ multi-task loss then fine-tune
\end{itemize} 

\noindent Pre-training consists of the initial training of our base CNN model and all of its layers.  We refer to \textit{fine-tuning} where the transfer learning occurs; this could entail freezing weights in the convolutional layers or not.  The sections that follow elaborate on each experiment.  

\subsubsection {Pre-train, Fine-tune (w/ and w/o weight-freezing; same task)}

Simple fine tuning without weight freezing begins with the pre-trained baseline model with a set of channels and proportion of the initial training set. As explained in the previous section, our fine tuning method uses an increasing sequence of proportions of the remaining data from the transfer learning partition, sections F1, F2, and F3. Section T is used for evaluation in all 3 rounds. See Figure \ref{fig:partition} for partition details.  

The sequence starts with using section F1, then combines sections F1 and F2 for the second round, with the final round combining sections F1, F2, and F3. Sections F1, F2, and F3 include trials from overlapping subjects; however, the pre-training dataset utilized entirely disjointed subjects (not present in test) – this is to simulate a realistic use-case where during per-subject training a base representation learned from other subjects can be used as a prior for fine-tuning a subject-specific classifier.  

During fine-tuning, the base learning rate was adjusted to 1e-4 (from 1e-3 used for pre-training) to ensure that pre-training representation knowledge was not “over-written” and to ensure convergence. We tried two approaches: one with no weight freezing and another with weight-freezing on all parameters except for the last two dense layers (i.e., the “frozen” network parameters were not updated during fine-tuning). 

\subsubsection {Pre-train then fine-tune (cross-task)}
Our approach to the cross-task experiments is essentially the same as the \textit{same task} (match/no-match EP) approach, except for the labels. For cross-task experiments, we pre-train our classifier using labels from a different task (alcoholic/nonalcoholic) and use match/no-match labels for fine tuning and evaluation.  

\subsubsection {Pre-train w/ auto-encoder then fine-tune}
This set of experiments attempts to pre-train using an unsupervised technique, then performs transfer learning in the standard supervised manner. Autoencoders are neural networks designed to reconstruct the original signal from a learnt “code-space” which notionally learns salient features from the data. This form of machine learning is referred to as \textit{representation learning}. Essentially, we are looking for useful intel from the auto-encoder during training and fine tuning.  

For the encoder, we used all layers from our pre-trained CNN up to the penultimate layer. The decoder consists of several fully-connected layers with layer normalization as a regularizer on all but the final fully-connected layer. The decoder is to be used only during pre-training. At transfer time, the decoder is discarded and the last two fully connected layers, initialized with Xavier weights \cite{glorot2010understanding} are attached to the network. 
% We utilized Xavier weights to avoid exploding or vanishing gradients by keeping the gradient norms closer to 1 by setting a layer’s weights to values chosen from a random uniform distribution bounded between
% \begin{equation}
% \label{eq:xavier_weights}
% \pm {\sqrt{6} \over \sqrt{n_i + n_{i+1}}},
% \end{equation}
% \noindent where $n_i$ is the number of incoming network connections to the layer, and $n_{i+1}$ is the number of outgoing network connections from that layer.  
The standard network architecture is then used at inference.

During pre-training of the auto-encoder, Mean Squared Error (MSE) loss was used. 
For each sample, given the $ith$ element, $y_i$, and $\hat y_i$ as the decoder's estimate of this element value ($n$ elements total where each element is the voltage at a specific window in time for a specific
channel), the per-sample loss becomes $MSE = \frac{1}{n}\sum_{i=1}^{n}(y_{i} - \tilde{y_{i}})^{2}$.

%The net loss over each minibatch is the sum of these losses per sample; see equation \ref{eq:mse}).

% \begin{equation}
% \label{eq:mse}
% MSE = \frac{1}{n}\sum_{i=1}^{n}(y_{i} - \tilde{y_{i}})^{2}
% \end{equation}

\subsubsection {Pre-train w/ Siamese loss then fine-tune}

 We pre-trained the CNN using a Siamese loss. Siamese networks are similar to metric learning insofar as they aim to optimize a deep network’s representation to place samples from the same class close to each other in projected space and samples from differing classes far away; we're attempting to get the network to maximize distances between match/non-match signals and minimize distances between match/match.   

The outputs of each network are typically in vector form. In our case there are two vectors, F1 and F2, corresponding to the penultimate layer of our stock CNN. We take the Euclidean distance between these vectors and then pass that through a sigmoid. Loss is evaluated in terms of binary cross entropy on the label. During fine-tuning, we use the shared weight network representation to initialize all of the weights on our model except for a final hidden layer which is initialized using an Xavier weight initialization.

The forward pass of the baseline network is replaced with a Siamese pass that essentially utilizes only a subset of the fully connected layers in the baseline CNN.  The output from the two subnetworks are two vectors, $F1$ and $F2$.  The Euclidean distance between the two vectors is calculated as $D= \sqrt{\sum_{i=1}^{n}\{F1_i-F2_i\}^2}$ and then passed through a sigmoid activation layer.  The loss from this sigmoid activation is computed using binary cross entropy.

%(see equation \ref{eq:EuclideanDistance}) and then passed through a sigmoid activation layer.  The loss from this sigmoid activation is computed using binary cross entropy.

% \begin{equation}
%  D= \sqrt{\sum_{i=1}^{n}\{F1_i-F2_i\}^2} 
% \label{eq:EuclideanDistance}
% \end{equation}

% $D$ is defined as the Euclidean distance between all outputs ($F1$ and $F2$) of the Siamese network.

\subsection{The Results}
We show a relevant subset of typical results as it's not feasible to display all 72 related charts in this paper.  All of our evaluations are in relation to the baseline training for the respective experimental group (match/no-match, HR/LR, and cross-task). 

\begin{figure}
\begin{tabular}{cc}
	%\includegraphics[width=56mm]{Images/roc_curves/transfer/transfer_experiments_binary_random_init_match_8_10.png} &  \hspace{-1.1cm}
	 %\includegraphics[width=80mm]{Images/roc_curves/transfer/transfer_experiments_binary_random_init_match_8_50.png} & \hspace{-.90cm}
	\includegraphics[width=40mm]{Images/roc_curves/transfer/transfer_experiments_binary_random_init_match_8_100.png}& \hspace{-.90cm}
	%\includegraphics[width=56mm]{Images/roc_curves/transfer/transfer_experiments_binary_random_init_match_12_10.png} &  \hspace{-1.1cm}
	 %\includegraphics[width=80mm]{Images/roc_curves/transfer/transfer_experiments_binary_random_init_match_12_50.png} & \hspace{-.90cm}
	%\includegraphics[width=40mm]{Images/roc_curves/transfer/transfer_experiments_binary_random_init_match_12_100.png} \\
	%\includegraphics[width=56mm]{Images/roc_curves/transfer/transfer_experiments_binary_random_init_match_60_10.png} &  \hspace{-1.1cm}
	 %\includegraphics[width=40mm]{Images/roc_curves/transfer/transfer_experiments_binary_random_init_match_60_50.png}& \hspace{-.90cm}
	\includegraphics[width=40mm]{Images/roc_curves/transfer/transfer_experiments_binary_random_init_match_60_100.png} \\
\end{tabular}
\caption{\label{fig:transferMatchRocs}ROC curves and AUC for match/no-match transfer baseline.  Each curve corresponds to the requisite fine-tuning partition as explained in Section \ref{sec:approach} and Figure \ref{fig:partition}.  The curves show performance using 60 channels vs. 8 channels.}
\end{figure}

\begin{figure}
\begin{tabular}{cc}
	%\includegraphics[width=56mm]{Images/roc_curves/transfer/transfer_experiments_binary_freeze_match_8_10.png} &  \hspace{-1.1cm}
	 %\includegraphics[width=65mm]{Images/roc_curves/transfer/transfer_experiments_binary_freeze_match_8_50.png} \hspace{-.90cm}
	%\includegraphics[width=65mm]{Images/roc_curves/transfer/transfer_experiments_binary_freeze_match_8_100.png} \\
	%\includegraphics[width=56mm]{Images/roc_curves/transfer/transfer_experiments_binary_freeze_match_12_10.png} &  \hspace{-1.1cm}
	 %\includegraphics[width=50mm]{Images/roc_curves/transfer/transfer_experiments_binary_freeze_match_12_50.png} \hspace{-.90cm}
	\includegraphics[width=40mm]{Images/roc_curves/transfer/transfer_experiments_binary_freeze_match_12_100.png}&
	\hspace{-.90cm}
	%\includegraphics[width=56mm]{Images/roc_curves/transfer/transfer_experiments_binary_freeze_match_60_10.png} &  \hspace{-1.1cm}
	 %\includegraphics[width=50mm]{Images/roc_curves/transfer/transfer_experiments_binary_freeze_match_60_50.png} \hspace{-.90cm}
	\includegraphics[width=40mm]{Images/roc_curves/transfer/transfer_experiments_binary_freeze_match_60_100.png} \\
\end{tabular}
\caption{\label{fig:transferMatchBinaryNoFreezeRocs}ROC curves and AUC for match/no-match pre-trained, fine-tuned, and with weight freezing.  The left shows performance with 12 channels while the right shows performance with 60 channels; notice the marginal improvement gained by increasing the feature space.}
\end{figure}

\begin{figure}
\begin{tabular}{cc}
	 %\includegraphics[width=65mm]{Images/roc_curves/transfer/transfer_experiments_random_init_alcoholic_8_50.png}
	 % \hspace{-.9cm} 
	  \includegraphics[width=40mm]{Images/roc_curves/transfer/transfer_experiments_random_init_alcoholic_8_100.png}&
	  \hspace{-.90cm}
	
	%\includegraphics[width=50mm]{Images/roc_curves/transfer/transfer_experiments_random_init_alcoholic_12_50.png}
	 %\hspace{-.9cm}  \includegraphics[width=50mm]{Images/roc_curves/transfer/transfer_experiments_random_init_alcoholic_12_100.png}
	
	%\includegraphics[width=50mm]{Images/roc_curves/transfer/transfer_experiments_random_init_alcoholic_60_50.png}
	 %\hspace{-.9cm} 
	  \includegraphics[width=40mm]{Images/roc_curves/transfer/transfer_experiments_random_init_alcoholic_60_100.png} \\		
\end{tabular}
\caption{\label{fig:transferAlcoholic}ROC curves and AUC for HR/LR baseline.  Each curve corresponds to the requisite fine-tuning partition as explained in Section \ref{sec:approach} and Figure \ref{fig:partition}.  The left shows performance training over 8 channels while the right shows performance with 60 channels.  Notice how this model seems stable across feature space dimensions.}
\end{figure}

\begin{figure}
\begin{tabular}{cc}
	 \includegraphics[width=40mm]{Images/roc_curves/transfer/transfer_experiments_siamese_no_freeze_alcoholic_8_50.png}& \hspace{-.90cm} \includegraphics[width=40mm]{Images/roc_curves/transfer/transfer_experiments_siamese_no_freeze_alcoholic_8_100.png} \\
	%\hspace{1cm} 
	%\includegraphics[width=50mm]{Images/roc_curves/transfer/transfer_experiments_siamese_no_freeze_alcoholic_12_50.png} \hspace{1cm}&  
	%\includegraphics[width=50mm]{Images/roc_curves/transfer/transfer_experiments_siamese_no_freeze_alcoholic_12_100.png} \\ 
	
	\includegraphics[width=40mm]{Images/roc_curves/transfer/transfer_experiments_siamese_no_freeze_alcoholic_60_50.png}&   \hspace{-.90cm} \includegraphics[width=40mm]{Images/roc_curves/transfer/transfer_experiments_siamese_no_freeze_alcoholic_60_100.png} \\		
\end{tabular}
\caption{\label{fig:transferAlcoholicSiameseNoFreeze}ROC curves and AUC for HR/LR with Siamese network, no weight freeze.  The top row shows performance with training over 8 channels while the bottom row shows performance over 60 channels.  The left column shows curves when trained with half the available data; the right shows performance using all of the available training data.  Notice how performance increases with the increase of either feature dimensions and/or the amount of training data.}
\end{figure}

\subsubsection {Match vs No-match}
This set of experiments is compared against the baseline CNN in Figure \ref{fig:transferMatchRocs}.  As can be seen from the ROC curves, the baseline starts out as a fairly poor performer and somewhat unstable across training data, channel, and tuning proportions.  The best performers were the simpler pretrained, fine-tuned CNN models.  These results represent a 16\% AUC improvement over the baseline, and a marginal improvement of 6\% over the results of the original experiments; however, with a much improved ROC curve, indicating improved performance and stability over every point (i.e. threshold) along the curve.  Performance difference between weight freezing and no-freeze is inconclusive. 

A word of caution here: choosing the “best” curves from Figure \ref{fig:transferMatchBinaryNoFreezeRocs} based on AUC alone would not be advisable; note that some of the curves cross.  In instances where ROC curves cross, you must consider the context of the classifier and which matters more to a given BCI system, a higher TPR or a lower FPR \cite{Hand-Mining-Tools}.

\subsubsection {High-risk vs Low-risk}
The curves for Siamese network without weight freezing show substantial performance over the match/no-match tasks, and show a moderate overall gain over the baseline.  Surprisingly, even the baseline performed strongly here (see Figure \ref{fig:transferAlcoholic}), outperforming the original CNN model in the previous experiments, as well as the RMDM model.  What's more, the worst performer for this category was the strongest performer for the match/no-match experiments: the pretrained, fine-tuned CNN model, performing no better than or below random chance.
Examine Figure \ref{fig:transferAlcoholicSiameseNoFreeze} for details.

\subsubsection {Cross-task}
All cross-task experiments were poor performers, coming in far below the baseline, slightly better than random chance, and unstable.  This was true regardless of training data proportion or number of channels used.  We plan to revise our experiments in the future to better evaluate our cross-tasks results.



==> sections/Interpretability.tex <==
\subsection {Interpretability}


\section {Conclusions}
Providing interpretable explainers can provide insight into what our models are learning.  For example, we may gain a much better understanding of why it's difficult to classify short latent EP (match/no-match) tasks by examining the explainers.  Notice how closely TP and TN resemble one another in the aggregate; spatial and temporal similarities are extremely narrow, and yet (astonishingly) transfer learning has enabled us to create a classifier that, not only performs reasonably well at this task, but generalizes extremely well, too.  In addition, we now have a better understanding of why classification for HR vs LW (clinical) performs much better than our match/no-match classifiers; the differences are more easily differentiated.  Understanding which channels or which areas of the head contribute most towards what our models learn may help in constructing specialized classifiers for use with specific BCI tasks and perhaps even with particular groups of users.

==> sections/Traditional_vs_Transfer.tex <==
\clearpage

\section{Traditional Vs. Transfer Experiments}\label{section:T-Vs-T}
For direct comparisons of traditional BCI classifiers with our transfer models we present the following results.  In each graph there are two solid ROC curves.  One curve represents the best transfer performer while the other the best traditional performer.  The dotted curves represent other models from the traditional experiments provided for additional contrast.  When examining these curves, take notice to how the performance progresses (or regresses) as dimensionality is increased. 

\begin{figure}[!htb]
	\begin{tabular}{cc}
		\includegraphics[width=56mm]{Images/roc_curves/tvt_alcoholic_detection_roc_60_10.png} &  \hspace{-1cm} 
		\includegraphics[width=56mm]{Images/roc_curves/tvt_alcoholic_detection_roc_60_100.png} \\
	\end{tabular}
	\caption{\label{fig:tvt_alcoholic_detection_60}Comparison of best performing traditional BCI classification with best transfer learning model for HR detection on 60 channels across various training proportions.  The solid red is the Siamese model with no weight freezing compared to the solid cyan representing the Riemannian Minimum Distance to Mean.  CNN and FFNN were provided for additional contrast.  Here you will notice how RMDM becomes unstable and degrades in performance when high dimensionality is introduced. }
\end{figure}


\begin{figure}[!htb]
	\begin{tabular}{cc}
		\includegraphics[width=56mm]{Images/roc_curves/tvt_match_detection_roc_60_10.png} &  \hspace{-1cm} 
		\includegraphics[width=56mm]{Images/roc_curves/tvt_match_detection_roc_60_100.png} \\
	\end{tabular}
	\caption{\label{fig:tvt_match_detection_60}Comparison of best performing traditional BCI classification with best transfer learning model for match detection on 60 channels across various training proportions.  The solid red is the binary model with weight freezing compared to the solid blue representing the our FFNN model.  LDA and RF were provided for additional contrast.}
\end{figure}

==> sections/rebuttal.tex <==
\section{Rebuttal}

\begin{small}

\subsection{Reviewer 1}

\noindent ``This article is a well-finished work with good illustrative and technical material.  The expediency of the presented list of references raises
doubts. We advise you to reduce the list of references."

\textbf{We had inadvertently included some references that we had read through in our research, but not directly referenced in the paper. We have removed extraneous references and cleaned up the reference section.}

\subsection{Reviewer 2}

\textbf{NOTE TO REVIEWER: We have re-written and better organized the related work and experiments/results sections.}

\noindent(1) ``EEG signal processing has known a huge interest during
the last decade, several models, processing and training
methodologies dedicated to EEG have been published. The
authors give a list of a part of the existing models but
did not analyze the related work to point out the context
in which this work is inserted. Moreover, several papers
concerning the use of transfer learning for EEG processing
(and other fields) are listed in the references but not
cited in the paper, have these references been used for
this paper? Related work section should be revised
including transfer learning approach for EEG."

\textbf{The rewrite of the related work section covers this.}

\noindent(2) ``In the dataset subsection, the employed dataset and the
data split with and without fine-tuning is presented. The
reviewer suspects that an inversion of references has been
made and that the reference [91] (not presenting an EEG
dataset) has been inverted with [1]. For the clarity of the
review, the reviewer will consider [1] when they will
mention the dataset. Moreover, as mentioned several times
in the paper, EEGs are signals that tend to be affected by
noise, however, no pre-processing steps are described? Have
the authors considered a specific signal pre-processing:
signal filtering, artefact removal method, etc? The
duration and sample frequency of the EEG signals are not
given which makes the paper very difficult to reproduce.
Finally, in the paper a study on the number of considered
electrodes has been made, however, the chosen 8/12 among
the 64 available is not mentioned in the paper either."

 \textbf{The reviewer is correct that the reference has been inverted. We have added the citation suggested by the reviewer as well as an additional citation by the same author which addresses the dataset in more detail. This is referenced in Sec. III-A. In this same section, we also mention:  ``For each trial, 1 second of EEG was collected at a 256 Hz sampling rate. Trials were
then filtered using a bandpass filter. In our experiments, we
use these filtered trials as is, with no re-sampling. While the
images were shown, EEG measurements were collected using
64 scalp electrodes (channels) with a standard 10/20 extended
spatial configuration [41]. Of the 64 channels, four serve as
reference and/or ground, so we conducted our experiments
using only the 60 non-reference channels or subsets thereof
according to the same 10/20 configuration.''}


\noindent(3) ``The authors proposed a dataset split based on subject
independent validation (i.e. training with N-i participants
and doing the test on the i remaining). However, it seems
that they only consider one split but did not re-iterate
the process to have a fair distribution of the participant
in each set (in the leave one subject cross-validation,
i.e. i=1, the process is reiterated for each participant
and the mean cross-validation for all the participant is
computed), this could affect the results depending on the
considered participant."

\textbf{The discussion of splits is clarified in Section III-A. The reviewer has a legitimate point that statistical aggregation using a leave one out regime does yield more robust results. However, the effect on results is specifically a concern with smaller numbers of subjects + trials. The dataset we utilize is relatively large compared to other datasets in the EEG space along both these veins and given that we utilized the same splits across experiments with consistent random seeds for weight initializations for our CNN model, the benchmarks offer actionable insights. Moreover, in setting the stage for future work with larger scale datasets, leave one out becomes an increasingly costly benchmark (e.g., leave one out is not used in large-scale computer vision evaluations b/c it is prohibitively expensive).} 

\noindent(4) 11The proposed ML and DL models seem straightforward
compared to existing works, is there any reason for this?
The proposed custom architecture by the authors is composed
of three 1D convolutions followed by a feed-forward neural
network, is there a particular choice for this
architecture? Why did not the authors consider channel-wise
convolution as it has been seen in more recent works [2]?" 

\textbf{We now elaborate in detail on the choice + rationale for architecture in Sec. III-B. We also reference the EEGNET paper, mentioning: ``A number of changes/refinements could be integrated, e.g., channel-wise
convolutions from [26], which could be an interesting future study. We note that we do not conduct a thorough architectural exploration in this paper, since the aim of our present study is to explore cross-subject transfer learning rather than perform detailed architectural comparisons".}

\noindent(5) ``It exists various approaches for transfer learning in
EEG [3], however in this work the authors only consider the
naive model fine-tuning. Is there any reason to choose this
method?"

\textbf{While it is correct that there are multiple approaches for transfer learning in EEG, we specifically focus on deep transfer learning on filtered EEG signals (i.e., no direct feature engineering), which already narrows down this subset. Within the broader deep learning literature, while there are an abundance of transfer learning methods, our approaches are relatively ubiquitous. In this paper, we are specifically interested in exploring the viability of cross-subject transfer. Exploring additional transfer learning techniques is a logical follow-up for future work.}

\noindent(6) ``In the experiments section, the authors refer to
results that are not written in the paper and the proposed
figure showing the results are too small to be analysed.
The fact that \textit{'We show a relevant subset of typical results
as it's not feasible to display all 72 related charts in
this paper'} is not eligible, the results could have been
separated into different subsections presenting the effect
of each modification: considered model, number of
electrodes, weight freezing, fine-tuning partition etc. The
results section has to be reworked."

\textbf{We agree that the experiments section in the originally submitted manuscript could have been clearer. Consequently, we re-wrote the entire section and specifically selected relevant results and added some results in tabular form.}

\subsection{Reviewer 3}

\noindent (1) ``The quality of images should be improved. The text is
not readable."

\textbf{The image quality has been improved and the images have been enlarged.}

\noindent(2) ``The view of an ideal BCI classifier does not seem
realistic. Not only the human brain is an ever-changing
model, but the EEG data collected from an individual during
a particular activity can vary because of emotions, mental
state, thoughts, etc. Finding a classifier that will be
all-encompassing of EEG data ever generated for an activity
does not seem feasible."

\textbf{We acknowledge that an “ideal BCI classifier” may never be attainable. However, we ultimately removed discussion of an “ideal BCI classifier”, as we believe that this distracts from the tangible results that this paper presents.}

\noindent (3) ``The statement (section III.A), \textit{'publicly available EEG
datasets of sufficient size and labeling that meets our
needs for this study'}, is very vague."

\textbf{Good point. We have elaborated on dataset requirements in Sec. III-A.
``However, training DL architectures on direct EEG data (as opposed to featurized data) requires additional labeled data and model regularization to avoid over-fitting [19]. This is an inherent limitation on performance achievable by current DL BCI classifiers"}

\noindent (4) ``Short hand notation should be used only after full forms
have been stated, eg, HR/LR"

\textbf{We have replace “HR/LR” with “High-Risk/Low-Risk”.}

\noindent (5) ``Dataset should be explained in brief. Mean age and
gender of participants, type of electrodes, device name,
tasks, duration for which data was collected, was any
preprocessing done?, etc."

\textbf{We explain the dataset in further detail in Sec. III-A and how we split it specifically for our experiments. We also provide additional citations which detail the dataset and collection process.}

\noindent (6) `` \textit{'Most BCI classifiers require
more data than what is typically provided to train
against.'} Support this with references."

\textbf{We have removed this phrasing and mention several times throughout the paper that BCI datasets are relatively small in the context of machine learning approaches and specifically deep learning approaches. Specifically, see Sec. 1 and Sec III-A.}

\noindent (7) ``What are T1, T2 and T3? Explain clearly."

\textbf{Dataset splits are now discussed in detail in Sec. III-A.}

\noindent (8) ``How was the selection of trials per subject for fine
tuning done? Was it random?"

\textbf{This is now discussed in Sec. III-A, Scenario 1 and III-A, Scenario 2.}

\noindent (9) ``\textit{'datasets of sufficient
size and labeling that meets our needs for this study'}.
This statement is vague and should be explained. How would
you quantify \textit{'needs for this study'}?"


\textbf{We have substantially re-written portions of this paper, consequently removing this vague phrasing. Please see Sec. I and Sec. II-A for discussion.}


\noindent (10) ``\textit{'Within each test, we started the test
with 8 channels, then 12 channels, and finally 60
channels'}. How were the channels selected? Was it random or
channels from nearby areas included, etc?"

\textbf{Chanel sampling/subsampling was conducted according to the 10/20 spatial configuration. We mention in Sec. III-A:``Of the 64 channels, four serve as reference and/or ground, so we conducted our experiments using only the 60 non-reference channels or subsets thereof according to the same 10/20 configuration."}

\noindent (11) ``The statement, \textit{'Selected channels correspond to typical
BCI configurations'} is very vague. Please elaborate."

\textbf{Please see above.}

\noindent (12) ``\textit{'One paper saw similar results on this type of EP
(P300), but surmised it was due to applying a prior spatial filter to
the data [96]. The authors’ conclusion is likely inaccurate, since our data has no such filter applied to it'}. Did the paper use the same dataset? If not then this statement does not seem fair."

\textbf{Out of fairness, we removed this assertion.}

\noindent (13) ``Many previous studies show that ensemble models perform
better than classical machine learning models for EEG. They
also show that deep learningmodels like 1D-CNN, LSTM
perform better with it than machine learning. The
contribution of the paper does not seem novel on that
front"

\textbf{This paper specifically addresses cross-subject deep transfer learning, but as the dataset and dataset configuration that we use have not been benchmarked in other literature, it is important to establish the relative performance of our approach with respect to other common ML classifiers including our tested ensemble methods (gradient boosting and random forests). We are encouraged that our findings are consistent with other literature in the field.}

\noindent(14) ``It does not seem fair to use more data for training for
transfer learning partition."

\textbf{We assume that this comment is in reference to the incorporation of the validation set from Scenario 1 into the training set of Scenario 2 (see the revised Fig. 1). This in no way biases the presented results, as it only affects the Scenario 2 experiments, which are consistent throughout and separated from Scenario 1 results.}

\noindent (15) ``\textit{'however, as the amount of data
increases other more robust classifiers catch up and then
surpass the performance of LDA.'} If other classifiers are
more robust than LDA then what is the reason for comparison
with LDA?"

\textbf{We have changed the phrasing of this within the paper. See Sec. IV-A. We compare with LDA as LDA is a commonly used classifer in the BCI space.}
\end{small}

==> zmtsbygsdtdvgdwnmvvjwjwcrrcpxhzs 2/README <==

August 26, 2015


IEEEtran is a LaTeX class for authors of the Institute of Electrical and
Electronics Engineers (IEEE) transactions journals and conferences.
The latest version of the IEEEtran package can be found at CTAN:

http://www.ctan.org/pkg/ieeetran

as well as within IEEE's site:

http://www.ieee.org/

For latest news, helpful tips, answers to frequently asked questions,
beta releases and other support, visit the IEEEtran home page at my
website:

http://www.michaelshell.org/tex/ieeetran/

Version 1.8b has a number of significant changes over the v1.8a release.
For a full history of changes, please read the file changelog.txt.
The most notable changes in this release include:

 1) Added new comsoc mode for the IEEE Communications Society.
    This mode (at present) only invokes the use of the newtxmath math fonts.
 
 2) Revised IEEEeqnarray column specifications to work with active " 
    (or other punctuation catcode changes) as with babel under the
    german or ngerman language modes. 
    Thanks to Stefan M. Moser for reporting this problem.

 3) Added \indexspace and other index related macros as newer versions of
    article.cls now do. These macros are needed to avoid an error when
    using the glossaries package.
    Thanks to Sebastian Nyberg for suggesting this change.

 4) Fixed odd/even page header font bug under compsoc mode and
    other page style code improvements.
    Thanks to Marco Paolieri for reporting this problem.

 5) Added hooks to allow for easy control of spacing above title.

 6) Added the \IEEEnoauxwrite command.
    Thanks to Sudarshan Mukherjee for suggesting this feature.


NOTE: Take care not to confuse the "comsoc" and "compsoc" class
options/modes as they are very different:

comsoc  ==> IEEE Communications Society
compsoc ==> IEEE Computer Society

The comsoc mode requires that an acceptable Times math font be available on
the LaTeX system. This requirement will be enforced by IEEEtran in comsoc
mode. Either the freely available newtxmath font by Michael Sharpe
http://www.ctan.org/pkg/newtx
(version 1.451, July 28, 2015 or later is recommended)
or the commercial MathTime font (e.g., mtpro2.sty) is acceptable.
See Section II-D (2.4) "Class Options - comsoc, compsoc, transmag" of
the IEEEtran HOWTO for more details.


Best wishes for all your publication endeavors,

Michael Shell
http://www.michaelshell.org/


********************************** Files **********************************

README                 - This file.

IEEEtran.cls           - The IEEEtran LaTeX class file.

changelog.txt          - The revision history.

IEEEtran_HOWTO.pdf     - The IEEEtran LaTeX class user manual.

bare_conf.tex          - A bare bones starter file for IEEE conference papers.

bare_conf_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         conference papers.

bare_jrnl.tex          - A bare bones starter file for IEEE journal papers.

bare_jrnl_comsoc.tex   - A bare bones starter file for IEEE Communications
                         Society journal papers.

bare_jrnl_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         journal papers.

bare_jrnl_transmag.tex - A bare bones starter file for IEEE Transactions
                         on Magnetics journal papers.

bare_adv.tex           - A bare bones starter file showing advanced
                         techniques such as conditional compilation,
                         hyperlinks, PDF thumbnails, etc. The illustrated
                         format is for an IEEE Computer Society journal paper.

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall the IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtran.cls, IEEEtran_HOWTO.pdf, bare_adv.tex,
                   bare_conf.tex, bare_conf_compsoc.tex, bare_jrnl.tex,
                   bare_jrnl_comsoc.tex, bare_jrnl_compsoc.tex,
                   bare_jrnl_transmag.tex
***************************************************************************


==> zmtsbygsdtdvgdwnmvvjwjwcrrcpxhzs 2/sections/Approach-Old.tex <==
\section{Approach}\label{sec:approach}

In Sec. \ref{sec:dataset}, we describe the dataset and data splits that we use under two evaluation scenarios: performance benchmarking (Scenario 1) and transfer learning evaluation (Scenario 2). We then describe our deep learning architecture and elaborate on our design rationale (Sec. \ref{sec:dl_model}). Next, we introduce traditional models against which we benchmark, under Scenario 1 to establish the viability of our deep learning architecture (Sec. \ref{sec:benchmark_models}). Finally, in Sec. \ref{sec:transfer_benchmark}, we discuss different transfer models which we evaluate under Scenario 2. 

\subsection{Evaluation Scenarios and Dataset}
\label{sec:dataset}

We re-partition the dataset introduced by Ingber et al. \cite{ingber1998statistical} according to two experimental scenarios. Scenario 1 is used to benchmark our deep learning architecture against traditional classifiers. Scenario 2 is used to evaluate different transfer learning approaches using our deep learning architecture.

\begin{figure}[h]
	%\vspace{-.70cm}
\centering
\includegraphics[scale=.40]{Images/DataPartition.png}
\caption{\label{fig:partition} Middle row: Scenario 1 Benchmark Partition dataset split. Bottom row: Scenario 2 Transfer Learning dataset split}
% \caption{\label{fig:partition} Data partitions used for our original benchmarking (middle row) and transfer learning experiments (bottom row).  F1, F2, and F3 (up to \%75 of the remaining data) are sections of data used for fine tuning, leaving section T (25\%) for testing.}
\end{figure} 

%\subsubsection{Scenario 1: Performance Benchmarking}
\noindent
{\bf Scenario 1: Performance Benchmarking}
We stratify our train, test, and validation partitions according to subjects, i.e., each partition contains all trials form selected subjects and no subject overlap exists between partitions. Subjects were sampled without replacement according to a uniform random distribution. Of the subjects, 70\% were assigned to the train set, 20\% were assigned to the test set, and 10\% were assigned to the validation set, which was used to establish hyperparameters.


\noindent
{\bf Scenario 2: Transfer Learning Evaluation}
%\subsubsection{Scenario 2: Transfer Learning Evaluation}
In Scenario 2, we combine the training and validation partitions from Scenario 1 into one monolithic partition for pre-training transfer learning variants of our deep learning architecture. We then split our test partition from Scenario 1 into four novel equal-sized partitions: three fine-tuning partitions (F1,F2,F3) and a single test partition (T). Note that these splits were stratified over trials, sampled according to a uniform random distribution, meaning that F1, F2, F3, and T have subject overlap with respect to one another, but contain no subject overlap with respect to the pre-training partition.  



% Our subject data is split into typical partitions: 70\% training set, 20\% test set, and 10\% validation set. It is important to note here that our 70/20/10 splits were based on subjects, thus there were no overlapping subjects across the data sets.  Subjects used in training were not present in the validation set, nor in the test set.  This ensured that we were able to properly evaluate cross-subject performance among our classifiers.  For our initial experiments with traditional BCI classifiers, we held the validation set aside to validate model hyperparameters.  When training our baseline CNN for transfer learning experiments, we combined the training and validation sets into a single training set (using roughly 80\% of the subject trials), and we used an increasing sequence of proportions of the remaining 20\% from the transfer learning partition (i.e. the remaining 20\% of subjects) for three rounds of fine tuning (F1 through F3), leaving the remaining data (T) for validation.  Refer to Figure \ref{fig:partition} for data partition details.

% The sequence starts with using 25\% (F1) of the entire tuning partition (F1, F2, F3, and T), then 50\% (F1+F2), and finally 75\% (F1+F2+F3); T (the last 25\%) was consistently withheld for evaluation.  It should be clearly noted here that unlike the benchmark partition, the transfer learning partition (specifically T1, T2, and T3) did include overlapping subjects for fine tuning, but with \textit{no overlapping subject trials}. For both groups of experiments we segmented experiment trials by incrementing the training data and number of channels used in the baseline model.  We performed 216 experimental tests: 54 cross-task + 81 match/no-match + 81 high-risk/low-risk.  \textit{Note that due to the number of experiments, we show a selection of typical performance graphs under section \ref{sec:experiments}, offering subsequent graphs via supplemental content upon request}.


\begin{figure*}[!b]
        \centering
        \subfloat[High-Risk/Low-Risk]{\label{fig:alcoholicFull}
        \includegraphics[width=0.45\linewidth]{Images/roc_curves/alcoholic_detection_roc_60_100.png}}
        \hfill
        \subfloat[Match/Non-Match]{\label{fig:matchFull}
        \includegraphics[width=0.45\linewidth]{Images/roc_curves/match_detection_roc_60_100.png}}
    \caption{Scenario 1 benchmarks trained using all 60 channels per trial and 100\% of the trials in the training set.}
\end{figure*}

\subsection{Deep Learning Model Architecture}
\label{sec:dl_model}

We design our deep learning model to be amenable to learning from relatively few EEG trials in comparison to data volumes seen in other domains, e.g., computer vision, NLP, etc. To this end, we introduce a convolutional architecture which explicitly sums responses from feature maps of varying temporal bandwidth (i.e., parallel convolutions), rather than hierarchically stacking and pooling feature maps. The rationale here is to explicitly enforce consideration of salient data at multiple time scales, rather than rely on multi-time scale data propagating through stacked convolutions. While the latter design could be effective, we surmise that it is also more prone to overfitting on EEG-scale datasets. A number of changes/refinements could be integrated, e.g., channel-wise convolutions from \cite{lawhern2018eegnet}, which could be an interesting future study. We note that we do not conduct a thorough architectural exploration in this paper, since the aim of our present study is to explore cross-subject transfer learning rather than perform detailed architectural comparisons.

Specifically, our model takes as input pre-specified channels from one second of EEG data (one trial) at a sampling-rate of 256 Hz. This corresponds to 256 input dimensions per-channel. The input data is fed to three separate convolutional layers in parallel with varying kernel sizes of 3, 7, and 11, respectively. Each convolutional layer contains 32-filters and padding is performed so that outputs are equidimensional. The outputs are then summed element-wise to enforce explicit consideration of variable temporal bandwidths during optimization.  Max pooling is then applied, using a kernel size of 2, and the convolutional outputs are then rasterized to a 1D vector of 4096 dimensions. This vector is then passed through a layer normalization layer (LNorm), followed by an exponential linear unit (ELU) activation, then two subsequent stacks of linear layers followed by LNorm and ELUs reduce the dimension first to 1024 then to 128. A final linear layer squashes the output to 1D and a sigmoid link function is applied. 

% We use a simple CNN model constructed for our benchmark experiments as our baseline.  All of our models are trained on nothing more than the raw EEG data in the dataset.  The layers for the network are configured as follows:

% \begingroup
% \tiny%
% \begin{center}
% 	\fbox{\begin{minipage}{\linewidth}
			
% 			\textbf{Part I:}\\
% 			\-\ Conv1d(64, 32, kernel\_size=(3,), stride=(1,), padding=(1,))\\
% 			\-\ Conv1d(64, 32, kernel\_size=(7,), stride=(1,), padding=(3,))\\
% 			\-\ Conv1d(64, 32, kernel\_size=(11,), stride=(1,), padding=(5,))\\
% 			\-\ MaxPool1d(kernel\_size=2, stride=2, padding=0, dilation=1)\\
% 			\textbf{Part II:}\\
% 			\-\ Sequential\textbf{(}
% 			\-\ (0): LayerNorm((4096,), eps=1e-05)\\
% 			\-\ (1): ELU(alpha=1.0)\\
% 			\-\ (2): Dropout(p=0.5, inplace=False)\\
% 			\-\ (3): Linear(in\_features=4096, out\_features=1024, bias=True)\\
% 			\-\ (4): LayerNorm((1024,), eps=1e-05, elementwise\_affine=True)\\
% 			\-\ (5): ELU(alpha=1.0)\\
% 			\-\ (6): Linear(in\_features=1024, out\_features=128, bias=True)\\
% 			\-\ (7): LayerNorm((128,), eps=1e-05, elementwise\_affine=True)\\
% 			\-\ (8): ELU(alpha=1.0)\\
% 			\-\ (9): Linear(in\_features=128, out\_features=1, bias=True)\\
% 			\-\ (10): Sigmoid()\textbf{)}
			
% 	\end{minipage}}
% 	\captionof{Model}{The baseline CNN model used throughout our experiments.\label{fg:A}}
% \end{center}
% \endgroup

We trained the network for 7 epochs (the point at which repeated testing showed stabilized loss), using a minibatch size of 128 trials over approximately 3,700+ trials per epoch. For the baseline model, we utilized a cross-entropy loss between the model output and the corresponding (binary) label during backpropagation.



% The network was trained over 7 epochs (the point at which repeated testing showed stabilized loss), each containing a batch size of 128 trials over approximately 3,700+ trials. We use cross entropy loss during back propagation, which is the negative log-likelihood over the entire data set, presuming some probabilistic model on label noise: 
% \begin{equation}
% \label{eq:crossentropy}
% E_{\mbox{\tiny entropy}} = -\sum_{c_=1}^M y_o,_c\log(p_o,_c),
% \end{equation} 
% Here, $M$ is the number of possible classes and $p$ is the predicted probability that the observation $o$ is class $c$. In our case, we only need to distinguish between two classes: EP and not EP.  Presuming a \textit{Bernoulli} model on label noise, this is equivalent to the binary cross entropy loss function:\textit{binary cross entropy}:
% \begin{equation}
% \label{eq:binarycrossentropy}
% E_{\mbox{\tiny entropy}} = -(y\log(p)+(1-y)log(1-p))
% \end{equation}


\subsection{Benchmark Comparison Models (Scenario 1)}
\label{sec:benchmark_models}

To justify the application of our convolutional neural network (CNN) architecture, we benchmark raw performance against a number of more traditional classifiers in Sec. \ref{sec:experiments} on the Scenario 1 test partition. These classifiers include a dense feed-forward neural network (FFNN), logistic regression (LR), a random forest ensemble (RF), linear discriminant analysis (LDA), and Riemannian minimum distance to mean (RMDM). Where applicable, hyperparameters were selected using a grid search over the Scenario 1 validation set.
% Include FFNN architecture if space

\subsection{Transfer Learning Comparison Models (Scenario 2)}
 \label{sec:transfer_benchmark}
  For our transfer learning evaluation, we train several variations of our base CNN architecture (cf. \ref{sec:dl_model}) on the Scenario 2 training partition. We then fine-tune on the Scenario 2 fine-tuning partitions (F1, F1+F2, F1+F2+F3), and assess performance on the test partition. Model variations include:
  \begin{itemize}
  \item Fine-tuning with reduced learning rate with and without weight freezing on all but the penultimate layer. 
  \item Cross-task pre-training and fine-tuning. 
  \item Pre-training with an auto-encoder layer and mean squared error (MSE) reconstruction loss attached to the penultimate layer of the base representation.
  \item Pre-training a Siamese version of the base representation under a contrastive loss.
  \end{itemize}
 
 
 %Finally, we discuss the the dataset that we employ in our  experiments (Sec. \ref{sec:experiments}) and crucially, the splits that we use to assess transfer learning performance (Sec. \ref{sec:dataset}).

% This section describes… 
% Model we use (ref A)
% Comparison models against which we benchmark in results 
% -	Why we’re doing the benchmark – establish some viability of the DL model, i.e., do we need deep learning?
% Dataset for transfer learning experiments
% -	Splits and partitions
%\subsection {The Baseline (CNN) Model}
 
 %The second group of experiments focuses on deep transfer learning experiments.  Transfer learning falls under a more general category of machine learning referred to as \textit{representation learning}\cite{goodfellow2016deep}.  We experiment with adapting some of the deep learning-oriented tasks from recent studies for our own purposes; this approach allows us to quickly analyze and identify techniques that are the most performant. We evaluate results from a number of experiments: 
% \begin {itemize}
% \itemsep-0.2em
% \item Pre-train then fine-tune (w/ and w/o weight-freezing; same task)
% \item Pre-train then fine-tune (cross-task)
% \item Pre-train w/ auto-encoder then fine-tune
% \item Pre-train w/ Siamese loss then fine-tune
% %\item Pre-train w/ multi-task loss then fine-tune
% \end {itemize} 

% Pre-training consists of the initial training of our base CNN model and all of its layers.  Fine-tuning is where the transfer learning happens.  For the base model, this entails either freezing weights in the convolutional layers or not.  The sections that follow elaborate on each experiment listed above. 





% An ideal BCI classifier would offer a high degree of scalability across large quantities of heterogeneous EEG data while requiring relatively little data and time to customize for any particular application. While this idealized classifier may not be fully realized, we explore how closely we might get to achieving such a model through 2 experiment groups: (1) experiments around traditional BCI classifiers and (2) experiments that unpack deep transfer learning and fine-tuning.





% An ideal BCI classifier would offer a high degree of scalability across large quantities of heterogeneous EEG data while requiring relatively little data and time to customize for any particular application. While this idealized classifier may not be fully realized, we explore how closely we might get to achieving such a model through 2 experiment groups: (1) experiments around traditional BCI classifiers and (2) experiments that unpack deep transfer learning and fine-tuning.

% %The ideal BCI classifier offers a high degree of scalability across large quantities of heterogeneous electroencephalographic data while requiring relatively little data and time to customize for any particular application. We explore how closely we might approach this idealistic model through 2 experiment groups: (1) experiments around traditional BCI classifiers and (2) experiments that unpack deep transfer learning and fine-tuning.

% The first group consists of experiments that pit a convolutional neural network (CNN) against a dense feed-forward neural network (FFNN) vs. logistic regression (LR) vs. random forest (RF) vs. linear discriminant analysis (LDA) vs. Riemannian minimum distance to mean (RMDM).  The second group of experiments focuses on deep transfer learning experiments.  Transfer learning falls under a more general category of machine learning referred to as \textit{representation learning}\cite{goodfellow2016deep}.  We experiment with adapting some of the deep learning-oriented tasks from recent studies for our own purposes; this approach allows us to quickly analyze and identify techniques that are the most performant. We evaluate results from a number of experiments: 
% \begin {itemize}
% \itemsep-0.2em
% \item Pre-train then fine-tune (w/ and w/o weight-freezing; same task)
% \item Pre-train then fine-tune (cross-task)
% \item Pre-train w/ auto-encoder then fine-tune
% \item Pre-train w/ Siamese loss then fine-tune
% %\item Pre-train w/ multi-task loss then fine-tune
% \end {itemize} 

% Pre-training consists of the initial training of our base CNN model and all of its layers.  Fine-tuning is where the transfer learning happens.  For the base model, this entails either freezing weights in the convolutional layers or not.  The sections that follow elaborate on each experiment listed above. 


% %\subsection{The Dataset}
% \subsection{Dataset Overview and Partitions}
% \label{sec:dataset}

% In order to study cross-subject transfer using classifiers which do not require engineered features, we require a dataset with sufficient subjects and samples to fit our proposed experimental models. As one of these is a deep learning model, this means that we need several thousand samples, ideally with samples distributed uniformly over subject trials.  %TODO: citation on the several thousand 
% We utilize a well-curated dataset from a large study that examined EEG correlates of genetic predisposition to alcoholism \cite{ingber1998statistical}. While the dataset is somewhat dated, it is one of the few publicly available EEG datasets that has the aforementioned characteristics that we require for this study.


% %We discovered a well-curated dataset from a large study that examined EEG correlates of genetic predisposition to alcoholism (1995). While the dataset is somewhat dated, it is one of the few publicly available EEG datasets of sufficient size and labeling that meets our needs for this study.  Several papers can be found that have used and/or describe the dataset chosen for this research: \cite{ingber1982statistical, shobeihi2006classification, bajwa2016neurokey, ccokyilmaz2011classification, lopes2004classification} 

% Our subject data is split into typical partitions: 70\% training set, 20\% test set, and 10\% validation set. It is important to note here that our 70/20/10 splits were based on subjects, thus there were no overlapping subjects across the data sets.  Subjects used in training were not present in the validation set, nor in the test set.  This ensured that we were able to properly evaluate cross-subject performance among our classifiers.  For our initial experiments with traditional BCI classifiers, we held the validation set aside to validate model hyperparameters.  When training our baseline CNN for transfer learning experiments, we combined the training and validation sets into a single training set (using roughly 80\% of the subject trials), and we used an increasing sequence of proportions of the remaining 20\% from the transfer learning partition (i.e. the remaining 20\% of subjects) for three rounds of fine tuning (F1 through F3), leaving the remaining data (T) for validation.  Refer to Figure \ref{fig:partition} for data partition details.

% The sequence starts with using 25\% (F1) of the entire tuning partition (F1, F2, F3, and T), then 50\% (F1+F2), and finally 75\% (F1+F2+F3); T (the last 25\%) was consistently withheld for evaluation.  It should be clearly noted here that unlike the benchmark partition, the transfer learning partition (specifically T1, T2, and T3) did include overlapping subjects for fine tuning, but with \textit{no overlapping subject trials}. For both groups of experiments we segmented experiment trials by incrementing the training data and number of channels used in the baseline model.  We performed 216 experimental tests: 54 cross-task + 81 match/no-match + 81 high-risk/low-risk.  \textit{Note that due to the number of experiments, we show a selection of typical performance graphs under section \ref{sec:experiments}, offering subsequent graphs via supplemental content upon request}.

% \begin{figure}[h]
% 	%\vspace{-.70cm}
% \centering
% \includegraphics[scale=.40]{Images/DataPartition.png}
% \caption{\label{fig:partition} Data partitions used for our original benchmarking (middle row) and transfer learning experiments (bottom row).  F1, F2, and F3 (up to \%75 of the remaining data) are sections of data used for fine tuning, leaving section T (25\%) for testing.}
% \end{figure} 





==> zmtsbygsdtdvgdwnmvvjwjwcrrcpxhzs 2/sections/Approach.tex <==
\section{Approach}\label{sec:approach}

In Sec. \ref{sec:dataset} we describe the dataset and data splits that we use under two evaluation scenarios: performance benchmarking (Scenario 1) and transfer learning evaluation (Scenario 2). We then describe our DL architecture and elaborate on our design rationale (Sec. \ref{sec:dl_model}). Next, we introduce traditional models against which we benchmark, under Scenario 1 to establish the viability of our DL architecture (Sec. \ref{sec:benchmark_models}). Finally, in Sec. \ref{sec:transfer_benchmark}, we discuss different transfer models which we evaluate under Scenario 2. 

\subsection{Evaluation Scenarios and Dataset}
\label{sec:dataset}

For our experiments, we re-partitioned an old but well-curated dataset \cite{ingber1997statistical,ingber1998statistical}. The original dataset includes 122 subjects from two groups: the first group contains 77 subjects with a high risk of alcoholic predisposition (``High-Risk") while the second group is a control group of 45 subjects with low risk of  alcoholism (``Low-Risk").  To elicit event-related potentials (ERPs), a delayed matching-to-sample task was used. For each subject, trials were conducted in which two images appeared in succession with a 1.6 second inter-stimulus interval. First, a random image (S1) from the set was displayed to the subject for 300ms. The image that followed was either a match to the first (S2 Match), or a different image altogether (S2 No Match). For each trial, 1 second of EEG was collected at a 256 Hz sampling rate. Trials were then filtered using a bandpass filter. In our experiments, we use these filtered trials as is, with no re-sampling. While the images were shown, EEG measurements were collected using 64 scalp electrodes (channels) with a standard 10/20 extended spatial configuration \cite{homan1987cerebral}. Of the 64 channels, four serve as reference and/or ground, so we conducted our experiments using only the 60 non-reference channels or subsets thereof according to the same 10/20 configuration. Match/Non-Match trials were balanced, with 120 trials per subject. All trials were randomized and balanced; one half of the trials contained matches, while the other half did not. 
%where recordings were segmented into 1-second windows which included 3.9ms epochs.

For our experiments, we utilize only the EEG taken from the query image (S2 Match/No-Match), labeling each EEG trial according to ``Match/Non-Match" and ``High-Risk/Low-Risk" respectively. We re-partitioned the dataset from ~\cite{ingber1997statistical} and \cite{ingber1998statistical} according to two experimental scenarios. Scenario 1 is used to benchmark our deep learning architecture against traditional classifiers. Scenario 2 is used to evaluate different transfer learning approaches using our deep learning architecture.

\begin{figure}[h]
	%\vspace{-.70cm}
\centering
\includegraphics[scale=.25]{Images/DataPartition.png}
\caption{\label{fig:partition} Dataset splits for Scenarios 1 (top) and 2 (bottom).}
% \caption{\label{fig:partition} Data partitions used for our original benchmarking (middle row) and transfer learning experiments (bottom row).  F1, F2, and F3 (up to \%75 of the remaining data) are sections of data used for fine tuning, leaving section T (25\%) for testing.}
\end{figure} 

%\subsubsection{Scenario 1: Performance Benchmarking}
\noindent
{\bf Scenario 1 -- Performance Benchmarking:}
We stratify our train, test, and validation partitions according to subjects, i.e., each partition contains all trials from selected subjects and no subject overlap exists between partitions. Subjects were sampled without replacement according to a uniform random distribution. Of the subjects, 70\% were assigned to the train set, 20\% were assigned to the test set, and 10\% were assigned to the validation set, which was used to establish hyperparameters.


\noindent
{\bf Scenario 2 -- Transfer Learning Evaluation:} In Scenario 2, we combine the training and validation partitions from Scenario 1 into one monolithic partition for pre-training transfer learning variants of our deep learning architecture. We then split our test partition from Scenario 1 into four novel equal-sized partitions: three fine-tuning partitions (F1,F2,F3) and a single test partition (T). Note that these splits were stratified over trials, sampled according to a uniform random distribution, meaning that F1, F2, F3, and T have subject overlap with respect to one another, but contain no subject overlap with respect to the pre-training partition.  

\begin{figure*}[!b]
        \centering
        \subfloat[High-Risk/Low-Risk]{\label{fig:alcoholicFull}
        \includegraphics[width=0.45\linewidth]{Images/roc_curves/alcoholic_detection_roc_60_100.png}}
        \hfill
        \subfloat[Match/Non-Match]{\label{fig:matchFull}
        \includegraphics[width=0.45\linewidth]{Images/roc_curves/match_detection_roc_60_100.png}}
    \caption{Scenario 1 benchmarks trained using all 60 channels per trial and 100\% of the trials in the training set.}
\end{figure*}

\subsection{Deep Learning Model Architecture}
\label{sec:dl_model}

We design our deep learning model to be amenable to learning from relatively few EEG trials in comparison to data volumes seen in other domains, e.g., computer vision, NLP, etc. To this end, we introduce a convolutional architecture which explicitly sums responses from feature maps of varying temporal bandwidth (i.e., parallel convolutions), rather than hierarchically stacking and pooling feature maps. The rationale here is to explicitly enforce consideration of salient data at multiple time scales, rather than rely on multi-time scale data propagating through stacked convolutions. While the latter design could be effective, we surmise that it is also more prone to overfitting on EEG-scale datasets. A number of changes/refinements could be integrated, e.g., channel-wise convolutions from \cite{lawhern2018eegnet}, which could be an interesting future study. We note that we do not conduct a thorough architectural exploration in this paper, since the aim of our present study is to explore cross-subject transfer learning rather than perform detailed architectural comparisons.

Specifically, our model takes as input pre-specified channels from one second of EEG data (one trial) at a sampling rate of 256 Hz. This corresponds to 256 input dimensions per-channel. The input data is fed to three separate convolutional layers in parallel with varying kernel sizes of 3, 7, and 11, respectively. Each convolutional layer contains 32-filters and padding is performed so that outputs are equidimensional. The outputs are then summed element-wise to enforce explicit consideration of variable temporal bandwidths during optimization.  Max pooling is then applied, using a kernel size of 2, and the convolutional outputs are then rasterized to a 1D vector of 4096 dimensions. This vector is then passed through a layer normalization layer (LNorm), followed by an exponential linear unit (ELU) activation, then two subsequent stacks of linear layers followed by LNorm and ELUs reduce the dimension first to 1024 then to 128. A final linear layer squashes the output to 1D and a sigmoid link function is applied. 

We trained the network for 7 epochs (the point at which repeated testing showed stabilized loss), using a minibatch size of 128 trials over approximately 3,700+ trials per epoch. For the baseline model, we utilized a cross-entropy loss between the model output and the corresponding (binary) label during backpropagation.


\subsection{Benchmark Comparison Models (Scenario 1)}
\label{sec:benchmark_models}

To justify the application of our convolutional neural network (CNN) architecture, we benchmark performance against a number of more traditional classifiers in Sec. \ref{sec:experiments} on the Scenario 1 test partition. These classifiers include a dense feed-forward neural network (FFNN), logistic regression (LR), a random forest (RF), gradient boosting (GB), linear discriminant analysis (LDA), and Riemannian minimum distance to mean (RMDM). Where applicable, hyperparameters were selected using a grid search over the Scenario 1 validation set.


\subsection{Transfer Learning Comparison Models (Scenario 2)}
 \label{sec:transfer_benchmark}
  For our transfer learning evaluation, we train several variations of our base CNN architecture (cf. \ref{sec:dl_model}) on the Scenario 2 training partition. We then fine-tune on the Scenario 2 fine-tuning partitions (F1, F1+F2, F1+F2+F3), and assess performance on the test partition. Model variations are as follows:

\noindent  
{\bf Baseline: } The CNN's weights were initialized using a Xavier initialization and the CNN was trained over F1, F1+F2, and F1+F2+F3 folds using a binary cross-entropy loss. The T fold was used for evaluation.

\noindent  
{\bf Variation 1: Same-Task Binary Pre-Training; Binary Fine Tuning: } The CNN was trained using the Scenario II pre-training partition, directly on labels, under a binary cross-entropy loss. Fine Tuning was performed over over F1, F1+F2, and F1+F2+F3 at a reduced learning rate. This experiment was repeated, freezing all weights up through the penultimate layer of the network.

\noindent  
{\bf Variation 2: Auto-Encoder Pre-Training; Binary Fine-Tuning: } Similar to Variation 1, except instead of pre-training with a binary cross-entropy loss, an the penultimate layer of the CNN served as the latent space of an auto-encoder. The auto-encoder was trained under a mean squared error (MSE) loss. The fine-tuning procedure was identical to that of Variation 1.

\noindent  
{\bf Variation 3: Siamese Pre-Training; Binary Fine-Tuning: } Similar to Variation 1, except instead of pre-training with a binary cross-entropy loss, a Siamese representation with contrastive loss was employed. The fine-tuning procedure was identical to that of Variation 1.

\noindent  
{\bf Variation 4: Cross-Task Binary Pre-Training; Binary Fine-Tuning: } Similar to Variation 1, except labels from one task were used in pre-training while labels from another task were used for fine-tuning and evaluation.


For Variations 1-3 we conducted our evaluation using both High-Risk/Low-Risk and Match/Non-Match labels. For Variation 4, the cross-task experiment, we used Match/Non-Match labels for pre-training and High-Risk/Low-Risk labels for fine-tuning.

  
  
  
  
%   \begin{itemize}
%   \item Fine-tuning with reduced learning rate with and without weight freezing on all but the penultimate layer. 
%   \item Cross-task pre-training and fine-tuning.
%   \item Pre-training with an auto-encoder layer and mean squared error (MSE) reconstruction loss attached to the penultimate layer of the base representation.
%   \item Pre-training a Siamese version of the base representation under a contrastive loss.
%   \end{itemize}
 
 

==> zmtsbygsdtdvgdwnmvvjwjwcrrcpxhzs 2/sections/Background.tex <==
\section{Background}
\label{sec:background}

BCI are built around one or more types of ERP buried in EEG, and when matched to tasks (i.e. a given context), these ERPs provide the basic building blocks for a BCI system. There are a number of challenges intrinsic to EEG data, for example, filtered (e.g., via a bandpass filter) EEG data is high-dimensional, has a low signal-to-noise ratio (SNR), and is \textit{highly} non-stationary. Evoked potentials (EPs) in EEG have an explicit dependence on the time variable (an EP is time-locked with the stimulus), making more input from the past necessary for classification and regression models. EEG contains biological artifacts such as eye blinks, muscle artifacts, and head movements~\cite{QuantitativeEEG}. 

Many of what we refer to as \textit{traditional} classifiers were applied to BCI before research focus shifted to deep learning models.  Many of these classifiers are based on liner models, such as variations of linear discriminant analysis (LDA), principal component analysis (PCA), and support vector machines (SVMs) -- including non-linear kernel SVMs~\cite{aloise2012comparison, krusienski2006comparison}. Bayesian approaches as well as clustering techniques, ensemble learning such as random forests (RF) and gradient boosting (GB), hidden Markov models (HMMs), and distance metrics are also considered \cite{lotte2007review, akram2015efficient, mainsah2015increasing, verschore2012dynamic, helmy2008p300, speier2014integrating, yger2016Riemannian}.  Most of these approaches include some degree of feature engineering.  We use some of these classifiers in our experimental comparisons; however, our work is particularly focused on deep transfer learning models.

\subsection{Deep Learning in BCI}

Deep learning (DL) both has and continues to achieve state-of-the-art performance in many areas of applied machine learning \cite{lecun2015deep,hestness2019beyond}, and consequently, recent BCI research leverages deep learning as well. Deep learning has the advantage that it can learn directly from filtered EEG data, rather than (necessarily) relying on SME-derived features.  Moreover, DL models are less sensitive to localization than traditional ML models \cite{lecun2015deep}. 

However, training DL architectures on direct EEG data (as opposed to featurized data) requires additional labeled data and model regularization to avoid over-fitting \cite{hestness2019beyond}. This is an inherent limitation on performance achievable by current DL BCI classifiers, as even the relatively large EEG dataset that we use in this paper consists ``merely" of thousands of trials from 122 subjects. For perspective, the Celeb-500k face recognition dataset \cite{cao2018celeb} consists of 50 million images from 500k individuals, which, according to Hestess et al.~\cite{hestness2019beyond} is still orders of magnitude too small to fully leverage DL.  However, as EEG sensors become more ubiquitous, cost effective, and ergonomic, we anticipate that labeled EEG dataset sizes will increase and performance of DL BCI models will ultimately improve as a result. 

There are a host of papers presenting various neural network and deep network architectures and applications towards improving BCI performance \cite{vavreka2017stacked, maddula2017deep, abdulhay2017investigation, liu2016time, soltanpour2016enhance, achanccaray2017p300, zafar2017electroencephalogram,lawhern2018eegnet}. 

\subsection{Transfer Learning in BCI}

Overwhelming evidence demonstrates that transfer learning techniques can increase performance over a multitude of tasks for almost any deep learning domain~\cite{tan2018survey}. As BCI has adopted deep learning a number of transfer learning techniques, including deep transfer learning techniques, have been pioneered \cite{giles2019subject, uran2019applying, ozdenizci2019transfer, wang2015review, atyabi2017reducing, wu2014transfer, rodrigues2019exploring, zanini2017transfer, zheng2016personalizing, he2017transfer, chai2017fast}. These works have tackled challenging aspects of transfer learning that are unique to EEG data, including varying electrodes, amplifiers, and stimulus modalities. In contrast to these, our work focuses on training a common base DL model in a generic multi-subject regime and adapting the model to novel subjects in a way that decreases per-subject data collection burden; we seek to generalize across filtered EEG without dependencies on specific feature engineering, stimulus modality, EEG hardware, tasks, or subjects.  
%(TL) 
%techniques can increase generalization across domains and tasks for almost any deep learning domain\cite{tan2018survey}. 
% Unpacking deep transfer learning for BCI was a natural progression once momentum behind deep learning for BCI increased, and at this point research using deep transfer learning for BCI is robust.  
% BCI is a particularly challenging domain in this regard, inherent difficulties with EEG notwithstanding.  One must consider that varying electrodes, amplifiers, and stimulus modalities exacerbate the challenges facing those who wish to port training from one BCI domain onto another.  Many transfer approaches, including deep transfer approaches now exist \cite{giles2019subject, uran2019applying, ozdenizci2019transfer, wang2015review, atyabi2017reducing, wu2014transfer, rodrigues2019exploring, zanini2017transfer, zheng2016personalizing, he2017transfer, chai2017fast}.

% In contrast to these, our work focuses on training a common base DL model in a generic multi-subject regime and adapting the model to novel subjects in a way that decreases per-subject data collection burden; we seek to generalize across filtered EEG without dependencies on specific feature engineering, stimulus modality, EEG hardware, tasks, or subjects.  

% \textbf{TODO: Chad}
% \begin{itemize}
% \item Brief citation of some traditional Transfer learning BCI works. --- OK
% \item Mention that we only care about deep transfer learning --- OK
% \item Discuss/survey deep transfer learning works that have been applied --- OK
% \item Explain what differentiates our work --- OK (but how much to cover in this section, probably needs more here)
% \end{itemize}

%There are a number of natural properties to EEG that present challenges for BCI classifiers.  EEG presents high dimensionality, has a very poor (low) signal-to-noise ratio (SNR) and is \textit{highly} non-stationary.  EPs in EEG have an explicit dependency on the time variable (it is time-locked with the stimulus), making more input from the past necessary for classification and regression models. EEG contains biological artifacts such as eye blinks, muscle artifacts, and head movements.  Research into the classification of ERP reveals that certain classifiers may perform better for specific types of ERP over others.  As a result there are many \textit{traditional} classifiers used in BCI \cite{krusienski2006comparison, aloise2012comparison, Theodoridis200991, lotte2007review, akram2015efficient, mainsah2015increasing, verschore2012dynamic, helmy2008p300, speier2014integrating}.

% \subsection{Deep Learning in BCI}

% Deep learning (DL) is setting state of the art performance in many major areas of machine learning today\cite{lecun2015deep}; therefore, as expected, we see more recent BCI-related papers have deep learning as a theme as well.  There are a host of papers presenting various neural network topologies and application towards improving BCI performance \cite{vavreka2017stacked, maddula2017deep, abdulhay2017investigation, liu2016time, soltanpour2016enhance, achanccaray2017p300, zafar2017electroencephalogram}.  What sets our work apart is how we assess and identify good performers for BCI and how these classifiers settle into specific types of BCI systems that can work with EP as well as a broader range of ERP; this work shows that there may not be a one-size-fits-all approach to covering EP and ERP applications with transfer learning.

==> zmtsbygsdtdvgdwnmvvjwjwcrrcpxhzs 2/sections/Conclusion.tex <==
\section{Conclusions}
\label{sec:conclusion}
Transfer learning can substantially augment performance and reduce training data requirements for BCI.  Comparing our baseline performance in Figure \ref{fig:transferMatchRocs} with our binary transfer results in Figure \ref{fig:transferMatchBinaryNoFreezeRocs} shows that even when using 1/3 of the transfer dataset to pre-train, our model substantially outperforms the baseline trained on the full transfer set by nearly 10\% in terms of area under the ROC curve. For the HR/LR results there are performance gains across all training sizes.

 The most prominent evidence brought to light here is that there is no single classifier in the group that performs well across tasks.  For short latent EP, our fine-tuned binary CNN model outperforms every other method we explored in this work, including our selected traditional BCI classifiers.  For long, sustained ERP patterns our Siamese approach outperformed all others by a large margin.  The performance trend continues upward as we increase the amount of data used for both training and fine-tuning, until we run out of data.



==> zmtsbygsdtdvgdwnmvvjwjwcrrcpxhzs 2/sections/ConclusionAndDiscussion.tex <==
\section{Discussion and Conclusions}
\label{sec:conclusion}

We have trained a deep learning CNN architecture across multiple heterogeneous subjects, and shown that cross-subject training  works effectively across two different tasks: detection of risk for alcoholism (High-Risk/Low-Risk) and detection of stimulus (Match/Non-Match). For the Match/Non-Match detection, the CNN outperforms all traditional benchmarks.

For High-Risk/Low-Risk detection, the CNN under-performs ensemble methods and Riemannian MDM classifier in terms of raw AU-ROC, but over-performs other benchmarks. In lower false positive rate (FPR) ranges, both the CNN and ensemble methods outperform Riemannian MDM. Note that the instability in the MDM ROC progressed as we increased the number of channels during our benchmark testing. Moreover, in contrast to the CNN, which seems to benefit from additional training data and number of electrodes, the Riemannian classifier performed better with fewer number of electrodes and its performance advantage over other classifiers was more pronounced in the low-data regime. This suggests that the CNN may scale more gracefully with increased data volumes than a Riemannian classifier, which is consistent with findings in the EEG literature \cite{lotte2018review,rodrigues2019exploring} wherein Riemannian classifiers perform well with small numbers of electrodes and do not scale well with larger input sizes. 

Most significantly, our transfer learning experiments demonstrate that by starting with a base representation trained across a multitude of heterogeneous subjects and transferring this representation to novel subjects, one can substantially reduce data requirements and/or enhance performance, even when the transfer representation is pre-trained on small data volumes.

For the High-Risk/Low-Risk transfer benchmark, we found that pre-training using a contrastive loss under a Siamese network regime, then fine-tuning over all weights using a reduced learning rate yielded the best transfer performance, while for the Match/Non-Match transfer benchmark, we found that freezing all weights up through the penultimate layer of a pre-trained model, trained on a binary cross-entropy loss, yielded best transfer performance. For the High-Risk/Low-Risk regime, the lack of transfer of the models that were pre-trained using a binary cross-entropy loss was unexpected. The lack of transfer under our cross-task training regime was additionally unexpected. We intend to examine cross-task transfer in more detail in future work.

These findings from our research may lead to benefits in consumer/clinical BCI applications, specifically as dataset sizes grow. With large datasets and consistent data collection protocols, the burden of data collection for training on a specific end-user could be dramatically reduced if not entirely eliminated for certain applications. Logical future directions of research include further exploration of cross-task transfer learning, pre-training across multiple optimization objectives, and refinements/improvements to selected deep transfer architectures.

==> zmtsbygsdtdvgdwnmvvjwjwcrrcpxhzs 2/sections/Discussion.tex <==
\section{Discussion}
\label{sec:discussion}

To better understand \textit{what} our models are learning we explored how to exploit interpretable explainers in novel ways.  Specifically, can we know how our models conjure their predictions, and can we determine whether or not those outputs are learning on features we would expect \cite{ribeiro2016should,doshi2017towards,molnar2019interpretable}?  Since there isn't a one-size-fits-all method towards \textit{interpretability}, we present evidence for our chosen approach for BCI EEG interpretability: integrated gradients (IG).    

Unlike metrics commonly used to analyze performance (accuracy, sensitivity, specificity and efficiency), the safety and trustworthiness of our models are rarely precisely quantified; however, these seemingly ancillary objectives may become very important in a given application and setting \cite{vellido2019importance,tjoa2019survey,lahav2018interpretable}.  For example, BCI holds much potential for use as a tool in clinical settings.  Such applications may aid clinicians and patients in the diagnosis and treatment of addiction disorders, learning disabilities, depression, dementia, epilepsy and more \cite{minguillon2017mobile, nakanishi2017detecting, al2017review,chatelle2018feasibility,pan2020prognosis,belkacem2020brain,ctarcuaapplication,roy2019deep}.  Under these circumstances, we must ensure the highest trust and reliability in our models.   

The authors of \cite {lundberg2017unified} provided evidence that many popular local interpretability methods, including the IG, Interpretable Model-Agnostic Explanations (LIME), and SHapley Additive exPlanations (SHAP) employ (essentially) the same explanation method: \textit{the additive feature attribution} (AFA) method.  AFA has three main properties which we review, local accuracy, missingness, and consistency.

Let \(f\) be the (complex) model we will interpret and \(g\) be the explainer model. \(f(x)\) is a prediction based on a single sample input \(x\).  Our explainers accept simplified input \(x'\) that map to the original input through the mapping function \(x=h_x\).  Local methods will (reasonably) ensure that \(g(z')\approx f(h_x (z'))\) whenever \(z'\approx x'\).  Keep in mind that because \(h_x\) is specific to the current input \(x\), \(h_x(x')=x\), despite \(x'\) containing less information than \(x\).

\begin{equation}
	\label{eq:additive_feature_attrib}
	\textrm{let }
	g(z') = \phi_0+\sum_{i_=1}^n \phi_i z'_i, 
\end{equation} 
where \(z'\in\{0,1\}^n\), \(n\) is the number of simplified input features, and \(\phi_i \in R\).
%\captionof{figure}{Additive feature attrribution methods have an explaination model that is a linear function of binary variables \cite {lundberg2017unified}}
These models all attribute an effect \(\phi_i\) to every feature, and summing these effects approximates the output of the original model prediction \(f(x)\). In short, the AFA method is simply a linear regression over a binary mask where deviations are guaranteed to be linear for local instances (think \textit{locality}).  This is also referred to as \textit{local accuracy}.  

\begin{equation}
	\label{eq:local_accuracy}
	f(x)=g(x') = \phi_0+\sum_{i_=1}^n \phi_i x'_i, 
\end{equation} 

In addition to this property, AFA method highlights two more ideal properties present in good interpretability models: property 2 is referred to as \textit{missingness}; it constrains certain features to have no attributed impact where 
\(x'\)=0.  
\begin{equation}
	\label{eq:additive_feature_prop2}
	x'=0 \Longrightarrow \phi_i = 0 
\end{equation} Property 3 is \textit{consistency}; the idea behind it states that an input's attribution should not decrease if a model changes so that some simplified input's contribution increases or stays the same regardless of other inputs, that input's attribution should not decrease \cite{lundberg2017unified,molnar2019interpretable}.

Let \(f(z')\)=\(f(h_x (z'))\) and \(z \backslash j'\) indicate that \(z'_j=0\) for any two models \(f and f'\) that satisfy:
\begin{equation}
	\label{eq:additive_feature_prop3}
	f'_x(z') - f'_x(z'_{\backslash j})\geq f_x(z') - f_x(z'_{\backslash j})
\end{equation}

for all input \(z' \in \{0,1\}^M\), then:
\(
\phi_j(f',x)\geq \phi_j(f,x)
\)

\subsection {Integrated Gradients (IG)}\label{section:IG}
%% intro to method, how applied here
In this seminal paper \cite{sundararajan2017axiomatic} the authors introduce IG as a self-evident (\textit{axiomatic}) method towards explainability; additive feature attribution (i.e. \textit{completeness}) can be viewed thusly: 
\textbf{\(\sum_{i_=1}^n IntegratedGrads_i(x) = F(x) - F(x')\)}, where \(x\) is the original input, \(x'\) is the baseline, and \(F: R^n\rightarrow [0,1]\) is the output of a neural network, assuming \(F : R^n\rightarrow R\) is \textit{differentiable almost everywhere}.

Formally, the integrated gradients defines the contribution of a given attribute, \(i\) for an input \(x\) and baseline \(x'\) thusly: let \(\frac{\partial F(x)}{\partial x_i}\) be the gradient of \(F(x)\) along the \(ith\) dimension. 
\begin{equation} \label{eq:IG}
	\begin{split}
		IntegratedGrads_i(x)::=\\ 
		(x_i-x'_i) \times \int_{\alpha=0}^1 \frac{\partial F(x'+\alpha \times (x-x'))}{\partial x_i}
	\end{split}
\end{equation}

Put another way, integrated gradients will aggregate the gradients along the inputs that fall on the (straight) line between the baseline and the input\cite{sundararajan2017axiomatic}.  This idea shows that IG is among a group of methods known as \textit{path methods}. Unlike many gradients methods used to interpret neural networks, IG avoids \textit{saturation} by integrating over a \textit{path}, which tells us, when scaled along this path, which attribute increased the output towards the correct classification\cite{sturmfels2020visualizing,sundararajan2017axiomatic}. 

\subsection{An Approach to Explainability}
 For our purposes we approach explainers as being a part of a decision support system (DSS) that may assist both technical and nontechnical persons assessing the performance of complex learning models by producing interpretable models that are much easier for humans to examine and assess.  We place the human in the loop so that we may learn the regions within the EEG signals where each classifier placed the greatest importance (highest weights).  Knowing this information may allow us to gain a better understanding of our data as well as our classifier models.  To our knowledge this work is the first to apply integrated gradients explainers to electroencephalography and BCI.  For a given model and threshold, we performed the following on the top performers for match/no-match and high-risk/low-risk:

\begin {enumerate}
\itemsep-0.25em
\item We start with the predictions (scores) related to the pretrained model.
\item For each examined sample (positive or negative) label, create an explainer:
\begin {enumerate}
\itemsep-0.25em
\item Evaluate the model using an allotment of test data.
\item Collect and rank all TP and TN scores using a chosen prediction threshold.
\item Aggregate the data samples across channels for the top N scores for each TP and TN
\item Obtain the feature attributions (i.e. weights) via integrated gradients (this results in a 2D array of IG weights for each channel and sample therein).
\item Using these weights, create a temporal \& spatial heat map that corresponds to each channel and its attributed factor.
\item Similarly, we use these weights to create a temporal and spatial dipole heat map that depicts the spatial and temporal contribution of each feature in the sample.
\end {enumerate}
\item We now have a way of examining what a classifier learns; we can better visualize from different perspectives what our models are learning.
\item We can examine each explainer to get an idea of which channels contribute positively or negatively to the overall prediction.
\end {enumerate}

\subsection{Interpreting the Explainers}

It is important that the reader does not discount the fact that examining information related to EEG \textit{requires} a certain level of knowledge in neuroscience, electroencephalography, BCI, or some combination of these topics.  Interpretability and related explainers are tools we seek to provide so that subject matter experts may evaluate what our models are learning.  We provide an interpretation of the explainers below so that readers without any background may examine what these explainers show.

In EP (match/no-match) we would expect the presence of early latent activity in EEG between 0 and 400 milliseconds after the stimulus is introduced to the subject; therefore, we should see some indication that our classifiers have learned some sort of representation of this early temporal activity.  Similarly, for sustained ERP (high-risk vs low-risk), we might see some sort of difference in how regions of the brain react to stimulus over time between high-risk and low-risk subjects.  According to our data analysis, normal progression should start towards the temporal region of the brain and eventually progress towards the frontal lobes.  We expect our models to have learned these differences in spatial progression between high-risk and low-risk subjects.  We fashioned our explainers to convey these details, assuming that they exist.

We created 3 types of visuals around our explainers: (1) A spatial dipole heat map representing weighted features as they relate to regions of the brain over an entire 1-second of time; represents spatial details only, (2) a joint temporal dipole heat map that represents weighted features as they progress over the length of a trial; also shows weights spatially and temporally for each channel, and (3) a channel heat map that shows how each feature's weighted contributions change over time within each channel.  We show several examples of these explainers and how we interpreted them.  Keep in mind that these images depict feature contributions (i.e. weighted features) towards a particular classification; they do not necessarily directly correspond to actual EEG amplitude.


\subsubsection{High Risk Vs. Low Risk Explainers}
Choosing a threshold of .51 we took all true positives (representing high-risk) and all true negatives (representing low-risk) and created explainers for each category.  Figures \ref{fig:tp_alcoholic_avg_all_dipole} and \ref{fig:SiameseAlcoholic_TP_ALL_joint_IG} depict the same things in different ways: all depict how EEG features contributed to high-risk classification.  Figures \ref{fig:tp_nonalcoholic_avg_all_dipole} and \ref{fig:SiameseAlcoholic_TN_ALL_joint_IG} all depict how EEG features contributed to low-risk classification.  

Comparing aggregated dipoles across subjects in Figures \ref{fig:tp_alcoholic_avg_all_dipole} and \ref{fig:tp_nonalcoholic_avg_all_dipole} provides us with the spatial differences between the two groups.  We can clearly see these differences when the images are juxtaposed.  These images tell us nothing about what was learned of ERP progression over time, but could be useful if we're not concerned with knowing those temporal details; this would depend on the application.

To gain a better understanding about what our Siamese transfer models learned about temporal progression, we can compare Figures \ref{fig:SiameseAlcoholic_TP_ALL_joint_IG} and \ref{fig:SiameseAlcoholic_TN_ALL_joint_IG}.  The biggest differences in the way the features contribute over time seem to be between the frontal lobes and the temporal lobe.  Low-risk subjects have large oscillatory feature swings starting in the temporal lobe that contribute to most of the activity within the first half of a trial, then shifting to the frontal lobes while high-risk subjects seem to show features related to the frontal lobes contributing more throughout the entire trial.  Interestingly enough, the low-risk group (also the control group) shows patterns that seem to jibe with what we'd expect to see in a normal subject.  High-risk is clearly different in this regard. 

If we change the temporal perspective slightly, we get yet another piece of information not readily visible in the first two representation.  Figures \ref{fig:SiameseAlcoholic_TP_ALL_joint_IG_heat} and \ref{fig:SiameseAlcoholic_TN_ALL_joint_IG_heat} depict temporal heat maps.  At first glance, these maps seem to introduce nothing but confusion; however, looking more closely at these two maps shows that is less “noise” in the low-risk map.  This could indicate that certain low-risk ERP features are more pronounced, overwhelming other less relevant features, leaving those features with barely any contribution (i.e. neutral weight).  This could be an indicator that some users of certain BCI systems may require systems that are better trained on more data from their respective clinically designated risk groups. 
%====== ERP Siamese Model Visuals ============

\begin{figure}[h]
	\centering
	\includegraphics[scale=.60]{Images/explainers/SiameseAlcoholic_TP_ALL_joint_IG_dipole_IG.png}
	\caption{\label{fig:tp_alcoholic_avg_all_dipole} A dipole heat map representing what our Siamese network learned over all high-risk tasks.  This image shows aggregated feature contributions (depicted through IG) across all TP high risk (alcoholic) subjects averaged across the entire length of a 1-second trial, showing which channels spatially contributed negatively (blue) or positively (red) towards the prediction.}
\end{figure}

\begin{figure}[h]
	\centering
	\includegraphics[scale=.27]{Images/explainers/SiameseAlcoholic_TP_ALL_joint_IG.png}
	\caption{\label{fig:SiameseAlcoholic_TP_ALL_joint_IG} A joint temporal dipole heat map representing what our Siamese network learned over all high-risk tasks.  This image shows aggregated feature contributions (depicted through IG) across all TP high risk (alcoholic) subjects through time over the entire length of a 1-second trial, showing which channels spatially and temporally contributed negatively (blue) or positively (red) towards the prediction.  Below the dipole maps we are able to follow the contributions of each EEG channel through time.}
\end{figure}

\begin{figure}[h]
	\centering
	\includegraphics[scale=.60]{Images/explainers/SiameseAlcoholic_TN_ALL_joint_IG_dipole_IG.png}
	\caption{\label{fig:tp_nonalcoholic_avg_all_dipole} A dipole heat map representing what our Siamese network learned over all \textbf{low-risk} tasks.  This image shows aggregated feature contributions (depicted through IG) across all low risk (non-alcoholic) subjects averaged across the entire length of a 1-second trial, showing which channels spatially contributed negatively (blue) or positively (red) towards the prediction.}
\end{figure}

\begin{figure}[h]
	\centering
	\includegraphics[scale=.25]{Images/explainers/SiameseAlcoholic_TN_ALL_joint_IG.png}
	\caption{\label{fig:SiameseAlcoholic_TN_ALL_joint_IG} A joint temporal dipole heat map representing what our Siamese network learned over all low-risk tasks.  This image shows aggregated feature contributions (depicted through IG) across all low risk (non-alcoholic) subjects through time over the entire length of a 1-second trial, showing which channels spatially and temporally contributed negatively (blue) or positively (red) towards the prediction.  Below the dipole maps we are able to follow the contributions of each EEG channel through time.}
\end{figure}

\begin{figure}[h]
	\centering
	\includegraphics[scale=.19]{Images/explainers/SiameseAlcoholic_TN_ALL_joint_IG_heat.png}
	\caption{\label{fig:SiameseAlcoholic_TN_ALL_joint_IG_heat} A temporal heat map representing what our Siamese network learned over all low-risk tasks.  This image shows aggregated feature contributions (depicted through IG) across all low risk (non-alcoholic) subjects through time over the entire length of a 1-second trial, showing which channels contributed negatively or positively towards the prediction.}
\end{figure}

\begin{figure}[h]
	\centering
	\includegraphics[scale=.19]{Images/explainers/SiameseAlcoholic_TP_ALL_joint_IG_heat.png}
	\caption{\label{fig:SiameseAlcoholic_TP_ALL_joint_IG_heat} A temporal heat map representing what our Siamese network learned over all high-risk tasks.  This image shows aggregated feature contributions (depicted through IG) across all TP high risk (alcoholic) subjects through time over the entire length of a 1-second trial, showing which channels contributed negatively or positively towards the prediction.}
\end{figure}

\subsection{Match Vs. No-Match Explainers}
Just as we did with the high-risk vs low-risk explainers for our Siamese model, we wish to gain some understanding into what our binary transfer model is learning about match/no-match trials.  Choosing a threshold of .51 we took all true positives (representing match) and all true negatives (representing no-match) and created explainers for each category. Unlike high-risk vs. low-risk, we expect to see most activity (i.e. most contributions) somewhere in the vicinity between 0 and 400 milliseconds.  Comparing the aggregate dipoles across subjects in Figures \ref{fig:BinaryMatch_TP_ALL_joint_IG_dipole} and \ref{fig:BinaryMatch_TN_ALL_joint_IG_dipole} provides us with the spatial differences between the two trials; however, we are much more interested in knowing if our model has learned the difference between P3a and P3b.

Contrasting Figures \ref{fig:BinaryMatch_TP_ALL_joint_IG} and \ref{fig:BinaryMatch_TN_ALL_joint_IG} we can clearly see that there is \textit{similar} progression of feature contributions in the temporal region between 0 and 400 milliseconds - just as we would expect from a classifier that was properly learning on early to mid latent EP features.  Notices how most features after 400 milliseconds have barely any positive contributions.  Our classifier is clearly learning the proper temporal aspects.   If we examine the differences in these contributions between match and no-match, we can see the differences made clearer there, too.  

The temporal heat maps in Figures \ref{fig:BinaryMatch_TP_ALL_IG_heat} and \ref{fig:BinaryMatch_TN_ALL_IG_heat} provide a better picture of which features in each channel contribute the most in the early temporal regions. We could us these sorts of heat maps to determine which channels we may omit to create less expensive, more portable BCI systems by cutting out channels that contribute less to the overall prediction coming from our classifiers. 

%====== EP Binary Model Visuals ============
\begin{figure}[h]
	\centering
	\includegraphics[scale=.19]{Images/explainers/BinaryMatch_TP_ALL_IG_heat.png}
	\caption{\label{fig:BinaryMatch_TP_ALL_IG_heat} A temporal heat map representing what our binary (CNN) network learned over all \textbf{match} tasks.  This image shows aggregated feature contributions (depicted through IG) across all TP match tasks through time over the entire length of a 1-second trial, showing which channels contributed negatively or positively towards the prediction.}
\end{figure}

\begin{figure}[h]
	\centering
	\includegraphics[scale=.19]{Images/explainers/BinaryMatch_TN_ALL_IG_heat.png}
	\caption{\label{fig:BinaryMatch_TN_ALL_IG_heat} A temporal heat map representing what our binary (CNN) network learned over all \textbf{no-match} tasks.  This image shows aggregated feature contributions (depicted through IG) across all TN match tasks through time over the entire length of a 1-second trial, showing which channels contributed negatively or positively towards the prediction.}
\end{figure}

\begin{figure}[h]
	\centering
	\includegraphics[scale=.60]{Images/explainers/BinaryMatch_TP_ALL_joint_IG_dipole.png}
	\caption{\label{fig:BinaryMatch_TP_ALL_joint_IG_dipole} A dipole heat map representing what our binary (CNN) network learned over all \textbf{match} tasks.  This image shows aggregated feature contributions (depicted through IG) across all TP match tasks averaged across the entire length of a 1-second trial, showing which channels spatially contributed negatively (blue) or positively (red) towards the prediction.}
\end{figure}

\begin{figure}[h]
	\centering
	\includegraphics[scale=.28]{Images/explainers/BinaryMatch_TP_ALL_joint_IG.png}
	\caption{\label{fig:BinaryMatch_TP_ALL_joint_IG} A joint temporal dipole heat map representing what our binary (CNN) network learned over all \textbf{match} tasks.  This image shows aggregated feature contributions (depicted through IG) across all TP match task through time over the entire length of a 1-second trial, showing which channels spatially and temporally contributed negatively (blue) or positively (red) towards the prediction.  Below the dipole maps we are able to follow the contributions of each EEG channel through time.}
\end{figure}

\begin{figure}[h]
	\centering
	\includegraphics[scale=.60]{Images/explainers/BinaryMatch_TN_ALL_joint_IG_dipole.png}
	\caption{\label{fig:BinaryMatch_TN_ALL_joint_IG_dipole} A dipole heat map representing what our binary (CNN) network learned over all \textbf{no-match} tasks.  This image shows aggregated feature contributions (depicted through IG) across all TN match tasks averaged across the entire length of a 1-second trial, showing which channels spatially contributed negatively (blue) or positively (red) towards the prediction.}
\end{figure}

\begin{figure}[h]
	\centering
	\includegraphics[scale=.25]{Images/explainers/BinaryMatch_TN_ALL_joint_IG.png}
	\caption{\label{fig:BinaryMatch_TN_ALL_joint_IG} A joint temporal dipole heat map representing what our binary (CNN) network learned over all \textbf{no-match} tasks.  This image shows aggregated feature contributions (depicted through IG) across all TN match task through time over the entire length of a 1-second trial, showing which channels spatially and temporally contributed negatively (blue) or positively (red) towards the prediction.  Below the dipole maps we are able to follow the contributions of each EEG channel through time.}
\end{figure}

==> zmtsbygsdtdvgdwnmvvjwjwcrrcpxhzs 2/sections/Experiments-Old.tex <==
\section{Experiments}
\label{sec:experiments}

The data includes 122 subjects with 2 groups: alcoholic predisposition (77 people) and control group (45 people). It is a balanced dataset in that trials were split roughly 50-50 between a form of popular go/no-go experiments often used in biological research with animal and human subjects (explained later as match/no-match trials). 64 scalp electrodes (channels) were used with a standard 10/20 extended spatial configuration. There were 120 trials per subject where recordings were segmented into 1-second windows which included 3.9ms epochs.  To elicit event-related potentials (ERPs), a delayed matching-to-sample task was used. Two images appeared in succession with a 1.6 second inter-stimulus interval. First, a random image (S1) from the set was displayed to the subject for 300ms. The image that followed was either a match to the first (S2 Match), or a different image altogether (S2 No Match).  All trials were randomized and balanced; one half of the trials contained matches, while the other half did not. 

\subsection{Model Benchmark Experiments}
 Classifiers were trained to detect two different pieces of information from the EEG dataset: (1) whether a given subject was part of the high-risk (HR) alcoholic group or the low-risk (LR) control group, and (2) whether a given subject trial resulted in a match or no-match scenario (labeled as 1 = match, 0 = no-match).

 We measured several aspects related to performance for each classifier: (1) which task a given classifier performed best at: (a) short elicited response patterns (match vs no-match) or (b) sustained ERP patterns (as in clinic classification or motor imagery), (2) which classifiers performed well with increased channels (which may increase both signal and noise), and (3) which classifiers performed well with less training data.

 We performed in total 126 experiments under 2 task groups: (1) match vs no-match and (2) high-risk (HR) vs low-risk (LR). There were 9 experiments performed for each of the 7 classifiers for each task group.  For each group we performed 3 sets of tests where each set used an increasing amount of the allocated training data (i.e. increased amount of trials for each subject).  Within each test we incrementally increased the number of channels used during the training process.  
 
 The tests progressed as follows: (1) Each test in each experiment started out using 10\% of the trials for each subject of the original 70\% training set, then the training set was incremented to 50\% of the trials, and finally 100\% of the subjects' trials. (2) Within each test, we started the test with 8 channels, then 12 channels, and finally 60 channels.  Selected channels correspond to typical BCI configurations.  (3) Performance for each classifier was recorded, ROC curves were compared relative to all other classifiers withing each experiment.  (4) Thresholds were evaluated to determine how well each classifier would perform under a given context (critical vs non-critical).

\subsection{Receiver Operating Characteristic (ROC) Curves}

We examine receiver operating characteristic (ROC) curves related to our experimental results for both the shape of the curves as well as the area under the curves (AUC).  To see additional ROC curves resulting from these experiments, please request our \textit{supplemental material}.
\begin{figure}
	\begin{tabular}{cc}
		%\includegraphics[width=46mm]{Images/roc_curves/match_detection_roc_8_10.png} &  \hspace{-1.1cm} 
		%\includegraphics[width=40mm]{Images/roc_curves/match_detection_roc_12_10.png}&  %\hspace{-1.1cm}\\
		%\hspace{-.90cm}
		%\includegraphics[width=40mm]{Images/roc_curves/match_detection_roc_60_10.png} \\
		%\includegraphics[width=46mm]{Images/roc_curves/match_detection_roc_8_50.png} &  \hspace{-1.1cm}
		 %\includegraphics[width=50mm]{Images/roc_curves/match_detection_roc_12_50.png} \hspace{-.90cm}
		%\includegraphics[width=50mm]{Images/roc_curves/match_detection_roc_60_50.png} \\
		%\includegraphics[width=46mm]{Images/roc_curves/match_detection_roc_8_100.png} &  \hspace{-1.1cm}
		\includegraphics[width=40mm]{Images/roc_curves/match_detection_roc_12_100.png}& %\hspace{-.90cm}
		\hspace{-.90cm}
		\includegraphics[width=40mm]{Images/roc_curves/match_detection_roc_60_100.png}\\ 
	\end{tabular}
\caption{\label{fig:matchRocs}ROC curves and AUC for match/no-match experimentation.  These curves show performance with 12 and 60 channels using 100\% of the available training data.}
\end{figure}

\begin{figure}
	\begin{tabular}{cc}
		%\includegraphics[width=46mm]{Images/roc_curves/alcoholic_detection_roc_8_10.png} &  \hspace{-1.1cm}
		\includegraphics[width=40mm]{Images/roc_curves/alcoholic_detection_roc_12_10.png}& % \hspace{-1.1cm}
		\hspace{-.90cm}
		\includegraphics[width=40mm]{Images/roc_curves/alcoholic_detection_roc_60_10.png}\\ 
		%\includegraphics[width=46mm]{Images/roc_curves/alcoholic_detection_roc_8_50.png} &\hspace{-1.1cm}
		 %\includegraphics[width=50mm]{Images/roc_curves/alcoholic_detection_roc_12_50.png} \hspace{-.90cm}
		%\includegraphics[width=50mm]{Images/roc_curves/alcoholic_detection_roc_60_50.png}\\
		%\includegraphics[width=46mm]{Images/roc_curves/alcoholic_detection_roc_8_100.png} &  \hspace{-1.1cm}
		\includegraphics[width=40mm]{Images/roc_curves/alcoholic_detection_roc_12_100.png} & %\hspace{-.90cm}
		\hspace{-.90cm}
		\includegraphics[width=40mm]{Images/roc_curves/alcoholic_detection_roc_60_100.png}\\ 
	\end{tabular}
\caption{\label{fig:alcoholichRocs}ROC curves and AUC for high-risk/low-risk experimentation.  The top row shows performance with 12 and 60 channels using only 10\% of the available training data.  The bottom row shows performance with 12 and 60 channels using 100\% of the available training data.}
\end{figure}

\subsection{Match Vs No-match Experiments}

This task group allowed us to experiment with how well our classifiers might perform in BCI designed for actionable EP.  These types of systems users to communicate with others, browse the internet, adjust environmental controls, flip lights on of off, etc..  Typically, they are built around visually evoked potentials or other early to mid-level latent responses such as P300.

 There are a few interesting things to note about our classifiers in in Figure \ref{fig:matchRocs}.  The Riemannian (RMDM) model did not perform at all for these sorts of tasks, performing no better than random chance; this was true for any test, regardless of the number of channels or the amount of training data.  Clearly, the RMDM classifier does not perform well as-is against raw EEG data where detecting short EP patterns is a requirement.  One paper saw similar results on this type of EP (P300), but surmised it was due to applying a prior spatial filter to the data \cite{congedo2019riemannian}.  The authors' conclusion is likely inaccurate, since our data has no such filter applied to it. 

When the amount of training data was low, LDA showed an interesting trend of increasingly better performance as the number of channels (i.e. feature space) increased.  LDA outperformed all other classifiers but gradient boosting (GB) when all 60 channels were used with the lowest amount of training data (see \ref{fig:matchRocs}).  LDA contends well with small amounts of high dimensional data; however, as the amount of data increases other more robust classifiers catch up and then surpass the performance of LDA.  This suggests that LDA does not generalize well across subjects and it doesn't contend well with increasing noise.  This suggests that LDA would require re-training for any user over a short period of time, since EEG for any subject is non-stationary over time.

Unlike LDA, the logistic regression (LR) model scaled better as the amount of training data was increased, showing good stability with 8 and 12 channels, but performance drops considerably with 60 channels.  This suggests that LR cannot scale well with high dimensional feature space, but generalizes across subjects where LDA cannot.  Examine the bottom row in Figure \ref{fig:matchRocs}.

Both of our ensemble methods, random forest (RF) and gradient boosting (GB) showed stable performance across all the tests.  Boosting shows a consistent edge in performance over random forest as well as a bit more stability, albeit a slight edge in both cases.  In fact, GB was outperformed only by our convolutional neural network (CNN) model when the full test set and all channels were in play; nevertheless, GB proved stable across all test. This suggests that ensemble approaches remain powerful, relevant models to BCI systems.  

Both feed-forward neural network (FFNN) and the convolutional neural network (CNN) were the overall top performers.  Overall, the CNN model outperforms our FFNN as the data and number of channels increases.  The FFNN shows some potential to perform slightly better on smaller quantities with a lesser feature space, showing that deep learning models have potential for good performance and generalization across subjects, noise (i.e. variance) and feature space across both temporal and spatial dimensions.  

\subsection{High-Risk Vs Low-Risk Experiment}
This series of tests evaluates how well our models might perform for BCI systems meant for clinical diagnostics or motor imagery.  These types of ERPs carry sustained patterns across longer periods of time, and are usually consistently cyclical in nature.  These ERPs can help clinicians identify pathological patterns in a subjects brain, or allow a user to move a prosthetic arm, hand, leg or wheelchair. Initially, we had expected results similar to the math/no-match experiment.  We refer you to Figure \ref{fig:alcoholichRocs}.

The RMDM model was the top performer in these tests among traditional classifiers.  While it's clear the RMDM (as-is) cannot contend with the shorter, noisier EP related tasks performed in the previous set of experiments, it shows here that RMDM does have an ability to draw out other patterns from ERP that none of the other classifiers could learn with these experiments.  RMDM remained stable and performs well regardless of how much training data was used.  In fact, performance increased when we stepped up from 8 channels to 12.  However, there are limits; RMDM quickly deteriorated, becoming less stable when incorporating all channels.  This demonstrates that there is clearly a limit to the dimensions in a given feature space.  This paper seems to back up this assumption: \cite{rodrigues2019exploring}.  The other classifiers performed poorly here, and showed a fair amount of instability.  

\subsection {Transfer Learning Experiments}

Given a source domain \(D_S\) and a (learning) task \(T_S\), a target domain \(D_T\) and its task \(T_T\), transfer learning seeks to improve the learning of the predictive target function \(f_T(\cdot)\) in \(D_T\) by using \textit{knowledge} in \(D_S\) and \(T_S\), assuming $(D_S \ne D_T), or (T_S \ne T_T)$.  For purposes of this study, a domain \(D\) is a \textit{subject} or number of subjects whose EEG data is used to train a specific model, and a task \(T\) is mapped to EP or ERP we wish to associate with actions related to context with a specific BCI.  

Here, evaluate results from a number of experiments: 
\begin {itemize}
\itemsep-.25em
\item Pre-train then fine-tune (w/ and w/o weight-freezing; same task)
\item Pre-train then fine-tune (cross-task)
\item Pre-train w/ auto-encoder then fine-tune
\item Pre-train w/ Siamese loss then fine-tune
%\item Pre-train w/ multi-task loss then fine-tune
\end{itemize} 

\noindent Pre-training consists of the initial training of our base CNN model and all of its layers.  We refer to \textit{fine-tuning} where the transfer learning occurs; this could entail freezing weights in the convolutional layers or not.  The sections that follow elaborate on each experiment.  

\subsubsection {Pre-train, Fine-tune (w/ and w/o weight-freezing; same task)}

Simple fine tuning without weight freezing begins with the pre-trained baseline model with a set of channels and proportion of the initial training set. As explained in the previous section, our fine tuning method uses an increasing sequence of proportions of the remaining data from the transfer learning partition, sections F1, F2, and F3. Section T is used for evaluation in all 3 rounds. See Figure \ref{fig:partition} for partition details.  

The sequence starts with using section F1, then combines sections F1 and F2 for the second round, with the final round combining sections F1, F2, and F3. Sections F1, F2, and F3 include trials from overlapping subjects; however, the pre-training dataset utilized entirely disjointed subjects (not present in test) – this is to simulate a realistic use-case where during per-subject training a base representation learned from other subjects can be used as a prior for fine-tuning a subject-specific classifier.  

During fine-tuning, the base learning rate was adjusted to 1e-4 (from 1e-3 used for pre-training) to ensure that pre-training representation knowledge was not “over-written” and to ensure convergence. We tried two approaches: one with no weight freezing and another with weight-freezing on all parameters except for the last two dense layers (i.e., the “frozen” network parameters were not updated during fine-tuning). 

\subsubsection {Pre-train then fine-tune (cross-task)}
Our approach to the cross-task experiments is essentially the same as the \textit{same task} (match/no-match EP) approach, except for the labels. For cross-task experiments, we pre-train our classifier using labels from a different task (alcoholic/nonalcoholic) and use match/no-match labels for fine tuning and evaluation.  

\subsubsection {Pre-train w/ auto-encoder then fine-tune}
This set of experiments attempts to pre-train using an unsupervised technique, then performs transfer learning in the standard supervised manner. Autoencoders are neural networks designed to reconstruct the original signal from a learnt “code-space” which notionally learns salient features from the data. This form of machine learning is referred to as \textit{representation learning}. Essentially, we are looking for useful intel from the auto-encoder during training and fine tuning.  

For the encoder, we used all layers from our pre-trained CNN up to the penultimate layer. The decoder consists of several fully-connected layers with layer normalization as a regularizer on all but the final fully-connected layer. The decoder is to be used only during pre-training. At transfer time, the decoder is discarded and the last two fully connected layers, initialized with Xavier weights \cite{glorot2010understanding} are attached to the network. 
% We utilized Xavier weights to avoid exploding or vanishing gradients by keeping the gradient norms closer to 1 by setting a layer’s weights to values chosen from a random uniform distribution bounded between
% \begin{equation}
% \label{eq:xavier_weights}
% \pm {\sqrt{6} \over \sqrt{n_i + n_{i+1}}},
% \end{equation}
% \noindent where $n_i$ is the number of incoming network connections to the layer, and $n_{i+1}$ is the number of outgoing network connections from that layer.  
The standard network architecture is then used at inference.

During pre-training of the auto-encoder, Mean Squared Error (MSE) loss was used. 
For each sample, given the $ith$ element, $y_i$, and $\hat y_i$ as the decoder's estimate of this element value ($n$ elements total where each element is the voltage at a specific window in time for a specific
channel), the per-sample loss becomes $MSE = \frac{1}{n}\sum_{i=1}^{n}(y_{i} - \tilde{y_{i}})^{2}$.

%The net loss over each minibatch is the sum of these losses per sample; see equation \ref{eq:mse}).

% \begin{equation}
% \label{eq:mse}
% MSE = \frac{1}{n}\sum_{i=1}^{n}(y_{i} - \tilde{y_{i}})^{2}
% \end{equation}

\subsubsection {Pre-train w/ Siamese loss then fine-tune}

 We pre-trained the CNN using a Siamese loss. Siamese networks are similar to metric learning insofar as they aim to optimize a deep network’s representation to place samples from the same class close to each other in projected space and samples from differing classes far away; we're attempting to get the network to maximize distances between match/non-match signals and minimize distances between match/match.   

The outputs of each network are typically in vector form. In our case there are two vectors, F1 and F2, corresponding to the penultimate layer of our stock CNN. We take the Euclidean distance between these vectors and then pass that through a sigmoid. Loss is evaluated in terms of binary cross entropy on the label. During fine-tuning, we use the shared weight network representation to initialize all of the weights on our model except for a final hidden layer which is initialized using an Xavier weight initialization.

The forward pass of the baseline network is replaced with a Siamese pass that essentially utilizes only a subset of the fully connected layers in the baseline CNN.  The output from the two subnetworks are two vectors, $F1$ and $F2$.  The Euclidean distance between the two vectors is calculated as $D= \sqrt{\sum_{i=1}^{n}\{F1_i-F2_i\}^2}$ and then passed through a sigmoid activation layer.  The loss from this sigmoid activation is computed using binary cross entropy.

%(see equation \ref{eq:EuclideanDistance}) and then passed through a sigmoid activation layer.  The loss from this sigmoid activation is computed using binary cross entropy.

% \begin{equation}
%  D= \sqrt{\sum_{i=1}^{n}\{F1_i-F2_i\}^2} 
% \label{eq:EuclideanDistance}
% \end{equation}

% $D$ is defined as the Euclidean distance between all outputs ($F1$ and $F2$) of the Siamese network.

\subsection{The Results}
We show a relevant subset of typical results as it's not feasible to display all 72 related charts in this paper.  All of our evaluations are in relation to the baseline training for the respective experimental group (match/no-match, HR/LR, and cross-task). 

\begin{figure}
\begin{tabular}{cc}
	%\includegraphics[width=56mm]{Images/roc_curves/transfer/transfer_experiments_binary_random_init_match_8_10.png} &  \hspace{-1.1cm}
	 %\includegraphics[width=80mm]{Images/roc_curves/transfer/transfer_experiments_binary_random_init_match_8_50.png} & \hspace{-.90cm}
	\includegraphics[width=40mm]{Images/roc_curves/transfer/transfer_experiments_binary_random_init_match_8_100.png}& \hspace{-.90cm}
	%\includegraphics[width=56mm]{Images/roc_curves/transfer/transfer_experiments_binary_random_init_match_12_10.png} &  \hspace{-1.1cm}
	 %\includegraphics[width=80mm]{Images/roc_curves/transfer/transfer_experiments_binary_random_init_match_12_50.png} & \hspace{-.90cm}
	%\includegraphics[width=40mm]{Images/roc_curves/transfer/transfer_experiments_binary_random_init_match_12_100.png} \\
	%\includegraphics[width=56mm]{Images/roc_curves/transfer/transfer_experiments_binary_random_init_match_60_10.png} &  \hspace{-1.1cm}
	 %\includegraphics[width=40mm]{Images/roc_curves/transfer/transfer_experiments_binary_random_init_match_60_50.png}& \hspace{-.90cm}
	\includegraphics[width=40mm]{Images/roc_curves/transfer/transfer_experiments_binary_random_init_match_60_100.png} \\
\end{tabular}
\caption{\label{fig:transferMatchRocs}ROC curves and AUC for match/no-match transfer baseline.  Each curve corresponds to the requisite fine-tuning partition as explained in Section \ref{sec:approach} and Figure \ref{fig:partition}.  The curves show performance using 60 channels vs. 8 channels.}
\end{figure}

\begin{figure}
\begin{tabular}{cc}
	%\includegraphics[width=56mm]{Images/roc_curves/transfer/transfer_experiments_binary_freeze_match_8_10.png} &  \hspace{-1.1cm}
	 %\includegraphics[width=65mm]{Images/roc_curves/transfer/transfer_experiments_binary_freeze_match_8_50.png} \hspace{-.90cm}
	%\includegraphics[width=65mm]{Images/roc_curves/transfer/transfer_experiments_binary_freeze_match_8_100.png} \\
	%\includegraphics[width=56mm]{Images/roc_curves/transfer/transfer_experiments_binary_freeze_match_12_10.png} &  \hspace{-1.1cm}
	 %\includegraphics[width=50mm]{Images/roc_curves/transfer/transfer_experiments_binary_freeze_match_12_50.png} \hspace{-.90cm}
	\includegraphics[width=40mm]{Images/roc_curves/transfer/transfer_experiments_binary_freeze_match_12_100.png}&
	\hspace{-.90cm}
	%\includegraphics[width=56mm]{Images/roc_curves/transfer/transfer_experiments_binary_freeze_match_60_10.png} &  \hspace{-1.1cm}
	 %\includegraphics[width=50mm]{Images/roc_curves/transfer/transfer_experiments_binary_freeze_match_60_50.png} \hspace{-.90cm}
	\includegraphics[width=40mm]{Images/roc_curves/transfer/transfer_experiments_binary_freeze_match_60_100.png} \\
\end{tabular}
\caption{\label{fig:transferMatchBinaryNoFreezeRocs}ROC curves and AUC for match/no-match pre-trained, fine-tuned, and with weight freezing.  The left shows performance with 12 channels while the right shows performance with 60 channels; notice the marginal improvement gained by increasing the feature space.}
\end{figure}

\begin{figure}
\begin{tabular}{cc}
	 %\includegraphics[width=65mm]{Images/roc_curves/transfer/transfer_experiments_random_init_alcoholic_8_50.png}
	 % \hspace{-.9cm} 
	  \includegraphics[width=40mm]{Images/roc_curves/transfer/transfer_experiments_random_init_alcoholic_8_100.png}&
	  \hspace{-.90cm}
	
	%\includegraphics[width=50mm]{Images/roc_curves/transfer/transfer_experiments_random_init_alcoholic_12_50.png}
	 %\hspace{-.9cm}  \includegraphics[width=50mm]{Images/roc_curves/transfer/transfer_experiments_random_init_alcoholic_12_100.png}
	
	%\includegraphics[width=50mm]{Images/roc_curves/transfer/transfer_experiments_random_init_alcoholic_60_50.png}
	 %\hspace{-.9cm} 
	  \includegraphics[width=40mm]{Images/roc_curves/transfer/transfer_experiments_random_init_alcoholic_60_100.png} \\		
\end{tabular}
\caption{\label{fig:transferAlcoholic}ROC curves and AUC for HR/LR baseline.  Each curve corresponds to the requisite fine-tuning partition as explained in Section \ref{sec:approach} and Figure \ref{fig:partition}.  The left shows performance training over 8 channels while the right shows performance with 60 channels.  Notice how this model seems stable across feature space dimensions.}
\end{figure}

\begin{figure}
\begin{tabular}{cc}
	 \includegraphics[width=40mm]{Images/roc_curves/transfer/transfer_experiments_siamese_no_freeze_alcoholic_8_50.png}& \hspace{-.90cm} \includegraphics[width=40mm]{Images/roc_curves/transfer/transfer_experiments_siamese_no_freeze_alcoholic_8_100.png} \\
	%\hspace{1cm} 
	%\includegraphics[width=50mm]{Images/roc_curves/transfer/transfer_experiments_siamese_no_freeze_alcoholic_12_50.png} \hspace{1cm}&  
	%\includegraphics[width=50mm]{Images/roc_curves/transfer/transfer_experiments_siamese_no_freeze_alcoholic_12_100.png} \\ 
	
	\includegraphics[width=40mm]{Images/roc_curves/transfer/transfer_experiments_siamese_no_freeze_alcoholic_60_50.png}&   \hspace{-.90cm} \includegraphics[width=40mm]{Images/roc_curves/transfer/transfer_experiments_siamese_no_freeze_alcoholic_60_100.png} \\		
\end{tabular}
\caption{\label{fig:transferAlcoholicSiameseNoFreeze}ROC curves and AUC for HR/LR with Siamese network, no weight freeze.  The top row shows performance with training over 8 channels while the bottom row shows performance over 60 channels.  The left column shows curves when trained with half the available data; the right shows performance using all of the available training data.  Notice how performance increases with the increase of either feature dimensions and/or the amount of training data.}
\end{figure}

\subsubsection {Match vs No-match}
This set of experiments is compared against the baseline CNN in Figure \ref{fig:transferMatchRocs}.  As can be seen from the ROC curves, the baseline starts out as a fairly poor performer and somewhat unstable across training data, channel, and tuning proportions.  The best performers were the simpler pretrained, fine-tuned CNN models.  These results represent a 16\% AUC improvement over the baseline, and a marginal improvement of 6\% over the results of the original experiments; however, with a much improved ROC curve, indicating improved performance and stability over every point (i.e. threshold) along the curve.  Performance difference between weight freezing and no-freeze is inconclusive. 

A word of caution here: choosing the “best” curves from Figure \ref{fig:transferMatchBinaryNoFreezeRocs} based on AUC alone would not be advisable; note that some of the curves cross.  In instances where ROC curves cross, you must consider the context of the classifier and which matters more to a given BCI system, a higher TPR or a lower FPR \cite{Hand-Mining-Tools}.

\subsubsection {High-risk vs Low-risk}
The curves for Siamese network without weight freezing show substantial performance over the match/no-match tasks, and show a moderate overall gain over the baseline.  Surprisingly, even the baseline performed strongly here (see Figure \ref{fig:transferAlcoholic}), outperforming the original CNN model in the previous experiments, as well as the RMDM model.  What's more, the worst performer for this category was the strongest performer for the match/no-match experiments: the pretrained, fine-tuned CNN model, performing no better than or below random chance.
Examine Figure \ref{fig:transferAlcoholicSiameseNoFreeze} for details.

\subsubsection {Cross-task}
All cross-task experiments were poor performers, coming in far below the baseline, slightly better than random chance, and unstable.  This was true regardless of training data proportion or number of channels used.  We plan to revise our experiments in the future to better evaluate our cross-tasks results.



==> zmtsbygsdtdvgdwnmvvjwjwcrrcpxhzs 2/sections/Experiments.tex <==




\section{Experiments}
\label{sec:experiments}

\subsection{Scenario 1: Performance Benchmark}

\noindent
{\bf Benchmark (All Data, All Channels): } Results for the High-Risk/Low-Risk benchmark are shown in Fig. \ref{fig:alcoholicFull}. Random forests (RF), Riemannian MDM (MDM), and Gradient Boosting (GB) slightly outperformed our CNN model, with the CNN outperforming the feedforward model (FFNN) and dramatically outperforming logistic regression (LR) and linear discriminant analysis (LDA). Results for the Match/Non-Match benchmark are shown in Fig. \ref{fig:matchFull}, where the CNN outperformed all other classifiers. In contrast to the High-Risk/Low-Risk regime, LDA performance increased, while MDM performance deteriorated.

\begin{figure*}[!t]
        \centering
        \subfloat[High-Risk/Low-Risk]{\label{fig:alcoholicPartialChannels}
        \includegraphics[width=0.45\linewidth]{Images/roc_curves/alcoholic_detection_roc_8_100.png}}
        \hfill
        \subfloat[Match/Non-Match]{\label{fig:matchPartialChannels}
        \includegraphics[width=0.45\linewidth]{Images/roc_curves/match_detection_roc_8_100.png}}
    \caption{Scenario 1 benchmarks trained and evaluated using a reduced set of 8 channels and 100\% of trials in the training set.}
\end{figure*}


\noindent
{\bf Effects of Channel Reduction:} In order to assess the effects of number of channels, we sub-selected only eight channels per trial to train and evaluate on. Channels were selected according to standard configuration. Results for High-Risk/Low-Risk detection are shown in Fig.
\protect\ref{fig:alcoholicPartialChannels}. Results for Match/Non-Match detection are shown in Fig. \protect\ref{fig:matchPartialChannels}. Notably, for High-Risk/Low-Risk, areas under Receiver Operating Characteristic (ROC) curves of all classifiers except MDM either remained roughly the same or were reduced; for MDM, performance significantly increased with lower input dimension. For Match/Non-Match, performance of all classifiers remained roughly the same or was reduced, with MDM still performing poorly. However, performance degradation across all classifiers was more graceful than under the High-Risk/Low-Risk regime.


\begin{figure*}[!t]
        \centering
        \subfloat[High-Risk/Low-Risk]{\label{fig:alcoholicPartialData}
        \includegraphics[width=0.45\linewidth]{Images/roc_curves/alcoholic_detection_roc_60_10.png}}
        \hfill
        \subfloat[Match/Non-Match]{\label{fig:matchPartialData}
        \includegraphics[width=0.45\linewidth]{Images/roc_curves/match_detection_roc_60_10.png}}
    \caption{Scenario 1 benchmarks, trained using 60 channels per trial and 10\% of the trials in the training set.}
\end{figure*}


\noindent
{\bf Effects of Data Reduction:} In order to assess sensitivity of our classifiers to data size,  we re-assessed the Scenario 1 benchmarks, training with only 10\% of the training trials. Trials were sampled according to a uniform random distribution. Results from the High-Risk/Low-Risk and Match/Non-Match experiments under this reduced data regime are shown in Fig. \ref{fig:alcoholicPartialData} and Fig. \ref{fig:matchPartialData} respectively. 

While performance generally deteriorated under both regimes compared with using all trials in train, the random forest was relatively unaffected for High-Risk/Low-Risk detection (net AUC slightly increased). Even with only 10\% of the training set, the CNN remained the top performing model in the Match/Non-Match regime.

\begin{figure*}[!t]
        \centering
        \subfloat[High-Risk/Low-Risk Baseline]{\label{fig:transferAlcoholicRocsBaseline}
        \includegraphics[width=0.45\linewidth]{Images/roc_curves/transfer/transfer_experiments_random_init_alcoholic_60_100.png}}
        \hfill
        \subfloat[High-Risk/Low-Risk Top Performer (Siamese Pre-Train)]{\label{fig:transferAlcoholicRocsSiamese}
        \includegraphics[width=0.45\linewidth]{Images/roc_curves/transfer/transfer_experiments_siamese_no_freeze_alcoholic_60_100.png}}
    \caption{Scenario 2 High-Risk/Low-Risk benchmarks.}
\end{figure*}

\subsection{Scenario 2: Transfer Learning Evaluation}
% \noindent
% {\bf High-Risk/Low-Risk Regime:} Baseline transfer results for High-Risk/Low-Risk evaluation are shown in Fig. \ref{fig:transferAlcoholicRocsBaseline}. The top performing transfer model was obtained via pre-training under a Siamese regime, then fine-tuning over the entire model at a reduced learning rate. Results from this model are shown in Fih. \ref{fig:transferAlcoholicRocsSiamese}.

% \noindent
% {\bf Match/Non-Match Regime:} Baseline results for the Match/Non-Match transfer evaluation are shown in Fig. \ref{fig:transferMatchRocsBaseline}. The top performing model was obtained by pre-training with a binary cross-entropy loss, freezing all weights up to the penultimate layer, then fine-tuning the unfrozen weights; see Fig. \ref{fig:transferMatchRocsFreeze}.

\begin{table}[!h]
	\caption{AU-ROCs High-Risk/Low-Risk}

	\label{tab:hr_lr_rocs}
	\begin{tabular}{lrrr}%
%		\toprule
		\textbf{Experiment}&\textbf{FT 0.25}&\textbf{FT 0.5}&\textbf{FT 0.75}\\
%		\midrule
		Baseline &0.683&0.802&0.829\\
		\textbf{Siamese (no freeze)}&\textbf{0.760}&\textbf{0.818}&\textbf{0.848}\\
        Siamese (freeze)&0.727&0.806&0.835\\
        Binary (freeze)&0.512&0.526&0.523\\
        Binary (no freeze)&{0.515}&{0.510}&{0.497}\\
        Auto-encoder (freeze)&0.655&0.712&0.749\\
        Auto-encoder (no freeze)&0.638&0.698&0.734\\

	\end{tabular}

\end{table} 

\begin{table}[!h]
	\caption{AU-ROCs Match/No Match}

	\label{tab:match_nonmatch_rocs}
	\begin{tabular}{lrrr}%
%		\toprule
		\textbf{Experiment}&\textbf{FT 0.25}&\textbf{FT 0.5}&\textbf{FT 0.75}\\
%		\midrule
		Baseline &0.608&0.712&0.659\\
		Siamese (no freeze)&0.660&0.703&0.771\\
        Siamese (freeze)&0.635&0.717&0.773\\
        \textbf{Binary (freeze)}&\textbf{0.787}&\textbf{0.796}&\textbf{0.801}\\
        {Binary (no freeze)}&{0.765}&{0.773}&{0.784}\\
        Auto-encoder (freeze)&0.568&0.642&0.673\\
        Auto-encoder (no freeze)&0.543&0.631&0.680\\
        
	\end{tabular}

\end{table}


Transfer results for the High-Risk/Low-Risk evaluation are shown in Table \ref{tab:hr_lr_rocs} in terms of area under each ROC (AU-ROC). The full ROC curves for the baseline model and top performing model are shown in Figs. \ref{fig:transferAlcoholicRocsBaseline} and \ref{fig:transferAlcoholicRocsSiamese} respectively. The top performing transfer model was obtained via pre-training under a Siamese regime, then fine-tuning over the entire model at a reduced learning rate. 

Transfer results for the Match/Non-Match evaluation are shown in Table \ref{tab:match_nonmatch_rocs} in terms of area under each ROC curve. The full ROC curves for the baseline model and top performing model are shown in Figs. \ref{fig:transferMatchRocsBaseline} and \ref{fig:transferMatchRocsFreeze} respectively. The top performing model was obtained by pre-training with a binary cross-entropy loss, freezing all weights up to the penultimate layer, then fine-tuning the unfrozen weights.

Transfer results for the Cross-Task transfer evaluation are shown in Table \ref{tab:match_nonmatch_rocs}. ROCs for these experiments are not shown as these models significantly under-performed the baseline.


\begin{figure*}[!b]
        \centering
        \subfloat[Match/Non-Match Baseline]{\label{fig:transferMatchRocsBaseline}
        \includegraphics[width=0.45\linewidth]{Images/roc_curves/transfer/transfer_experiments_binary_random_init_match_60_100.png}}
        \hfill
        \subfloat[Match/Non-Match Top Performer (Frozen Weights from Pre-Training Through Penultimate Layer)]{\label{fig:transferMatchRocsFreeze}
        \includegraphics[width=0.45\linewidth]{Images/roc_curves/transfer/transfer_experiments_binary_freeze_match_60_100.png}}
    \caption{Scenario 2 Match/Non-Match benchmarks.}
\end{figure*}



\begin{table}
	\caption{AU-ROCs Cross-Task}

	\label{tab:cross-task_rocs}
	\begin{tabular}{lrrr}%
%		\toprule
		\textbf{Experiment}&\textbf{FT 0.25}&\textbf{FT 0.5}&\textbf{FT 0.75}\\
%		\midrule
        Binary cross-task (freeze)&0.581&0.597&0.617\\
        Binary cross-task (no freeze)&0.617&0.634&0.665\\
        
	\end{tabular}

\end{table}

==> zmtsbygsdtdvgdwnmvvjwjwcrrcpxhzs 2/sections/Interpretability.tex <==
\subsection {Interpretability}


\section {Conclusions}
Providing interpretable explainers can provide insight into what our models are learning.  For example, we may gain a much better understanding of why it's difficult to classify short latent EP (match/no-match) tasks by examining the explainers.  Notice how closely TP and TN resemble one another in the aggregate; spatial and temporal similarities are extremely narrow, and yet (astonishingly) transfer learning has enabled us to create a classifier that, not only performs reasonably well at this task, but generalizes extremely well, too.  In addition, we now have a better understanding of why classification for HR vs LW (clinical) performs much better than our match/no-match classifiers; the differences are more easily differentiated.  Understanding which channels or which areas of the head contribute most towards what our models learn may help in constructing specialized classifiers for use with specific BCI tasks and perhaps even with particular groups of users.

==> zmtsbygsdtdvgdwnmvvjwjwcrrcpxhzs 2/sections/Introduction.tex <==
\section{Introduction}
\label{sec:intro}


% Things to mention here...

% 1. Traditional BCI has involved very problem specific approaches, features, data collection, etc.

% 2. Notable exceptions discussed in background but they do not generalize 

% 3. Our approach utilizes combinations of:
%	a) learning from raw data 
%	b) transfer learning 
%	c) interpretability, inspired from vision domains

 BCI captures, measures and records brain function via brainwaves and relates those measurements to some sort of external classification, action, or task~\cite{wolpaw2012brain, EEG_Signal_Processing, QuantitativeEEG}.  These recordings, typically captured via electrodes placed externally over the scalp, are referred to as \textit{electroencephalography} (EEG). EEG contains \textit{event-related potentials} (ERP) -- measured brain responses that are generated by the brain's cognitive, sensory, or motor functions.  ERP may be time-locked with both sensory and cognitive neuronal processes and then turned into executable or labeled actions by the BCI.  BCI systems rely on classifiers designed to identify and classify ERP related to tasks within the context of a specific system design.

At the time of this writing consumer and clinical BCI viability remains low, due to problematic aspects associated with EEG data: EEG is noisy, non-linear and highly non-stationary~\cite{EEG_Signal_Processing, QuantitativeEEG}, and ERP varies spatially and temporally between different mental tasks as well as across users~\cite{chiou2016spatial, li2020transfer}. Moreover, collection can be time-consuming, tedious, and error-prone sometimes leading to a dirth of available data in comparison to other machine learning domains, e.g., computer vision datasets often consist of millions to hundreds of millions of images, whereas even large EEG datasets consist of only a few thousand trials. 
% citation for cv dataset sizes vs eeg dataset sizes

In consumer/clinical application, the BCI community tends to address these challenges via manually crafted features constructed with subject matter expertise. % citation on SME features used for consumer/clinical BCI applications
This featurization approach makes extracting relevant signal and fitting classifiers feasible on relatively small datasets for a specific subject and a specific task. However, such features also introduce a high degree of inductive bias~\cite{goyal2020inductive} which may attenuate relevant responses associated with other tasks, including cross-subject correlation. Our approach utilizes a deep learning architecture, which operates directly on filtered EEG signals, yet is simultaneously engineered for fitting on EEG-scale datasets. Our approach is thus application-agnostic. 

We hypothesize that our approach 1) can learn a representation which works well across subjects in generic form and 2) can consequently be domain-adapted to novel subjects with a specific BCI application under a transfer learning regime. This work makes the following contributions:

\begin {itemize}
\itemsep-0.25em

\item Novel evaluation of transfer learning approaches towards generalization techniques that allow for simplified and shortened classifier training specific to EEG. 

\item Evaluation of traditional EP BCI classifiers with respect to performance on filtered EEG data (i.e. no hand-crafted features). 

\item Evaluation of EP classifiers with respect to generalization potential across subjects and tasks.
\end {itemize}




% small datasets that do not necessarily generalize well across subjects as well as features which potentially are ill-suited to generalizing across subjects have led to EEG deployments which do necessarily consider cross-subject correlations and ways that they could be used to reduce data collection-burden per-subject. Our approach specifically aims to advance cross-subject transfer and reduce data collection requirements per-subject 



% Inductive Bias = Model Justification

% Want to discuss tradeoffs of high-vs-low inductive bias and provide citations:
% 	-high inductive bias advantage: allows fitting based on noisy and small datasets
% 	-disadvantage: presumes presence of relevant response w/in the data but might ignore signal that it's not looking for
% 	- feature-based models have intrinsically high inductive bias; but especially when correlating across subjects, there is concern that they might ignore relevant data
% 	- models that learn from raw data often require enormous datasets to work well, which precludes EEG applications

% We propose an approach to learn from raw data, in a deep learning regime, yet bake *enough* inductive bias into our model that it learns quickly and efficiently from from a feasible-to-collect EEG dataset (i.e., several thousand vs several million+ samples) in other deep learning domains.

% Transfer Learning

% small datasets that do not necessarily generalize well across subjects as well as features which potentially are ill-suited to generalizing across subjects have led to EEG deployments which do necessarily consider cross-subject correlations and ways that they could be used to reduce data collection-burden per-subject. Our approach specifically aims to advance cross-subject transfer and reduce data collection requirements per-subject 




%There are problematic aspects buried deep within the nature of EEG: it's noisy, non-linear and highly non-stationary\cite{EEG_Signal_Processing, QuantitativeEEG} and collection can be time-consuming, tedious, and error-prone sometimes leading to a dirth of available data.

% Additionally, ERP varies spatially and temporally between different mental tasks as well as across users\cite{chiou2016spatial, li2020transfer}.
% Consequently, classifiers often rely on feature-engineered models with intrinsically stronger inductive biases, rather than learning directly from the signal itself; 
% therefore, traditional classifiers for BCI offer little  scalability across tasks or users\cite{2017arXiv170707935M}. 
% This work explores classifiers aimed to better generalize across EP embedded in human EEG data by operating closer to the raw signal.

% At the time of this writing consumer and clinical BCI viability remains low.  There are problematic aspects buried deep within the nature of EEG: it's noisy, non-linear and highly non-stationary\cite{EEG_Signal_Processing, QuantitativeEEG}.  Most BCI classifiers require more data than what is typically provided to train against.  ERP varies spatially and temporally between different mental tasks as well as across users\cite{chiou2016spatial, li2020transfer}.  In addition, traditional classifiers for BCI do not offer scalability across tasks or users\cite{2017arXiv170707935M}.  The major thrust behind this work is the exploration of classifiers that seem better suited to generalizing across EP embedded in human EEG data.






==> zmtsbygsdtdvgdwnmvvjwjwcrrcpxhzs 2/sections/Traditional_vs_Transfer.tex <==
\clearpage

\section{Traditional Vs. Transfer Experiments}\label{section:T-Vs-T}
For direct comparisons of traditional BCI classifiers with our transfer models we present the following results.  In each graph there are two solid ROC curves.  One curve represents the best transfer performer while the other the best traditional performer.  The dotted curves represent other models from the traditional experiments provided for additional contrast.  When examining these curves, take notice to how the performance progresses (or regresses) as dimensionality is increased. 

\begin{figure}[!htb]
	\begin{tabular}{cc}
		\includegraphics[width=56mm]{Images/roc_curves/tvt_alcoholic_detection_roc_60_10.png} &  \hspace{-1cm} 
		\includegraphics[width=56mm]{Images/roc_curves/tvt_alcoholic_detection_roc_60_100.png} \\
	\end{tabular}
	\caption{\label{fig:tvt_alcoholic_detection_60}Comparison of best performing traditional BCI classification with best transfer learning model for HR detection on 60 channels across various training proportions.  The solid red is the Siamese model with no weight freezing compared to the solid cyan representing the Riemannian Minimum Distance to Mean.  CNN and FFNN were provided for additional contrast.  Here you will notice how RMDM becomes unstable and degrades in performance when high dimensionality is introduced. }
\end{figure}


\begin{figure}[!htb]
	\begin{tabular}{cc}
		\includegraphics[width=56mm]{Images/roc_curves/tvt_match_detection_roc_60_10.png} &  \hspace{-1cm} 
		\includegraphics[width=56mm]{Images/roc_curves/tvt_match_detection_roc_60_100.png} \\
	\end{tabular}
	\caption{\label{fig:tvt_match_detection_60}Comparison of best performing traditional BCI classification with best transfer learning model for match detection on 60 channels across various training proportions.  The solid red is the binary model with weight freezing compared to the solid blue representing the our FFNN model.  LDA and RF were provided for additional contrast.}
\end{figure}

==> zmtsbygsdtdvgdwnmvvjwjwcrrcpxhzs 2/sections/rebuttal.tex <==
\section{Rebuttal}

\begin{small}

\subsection{Reviewer 1}

\noindent ``This article is a well-finished work with good illustrative and technical material.  The expediency of the presented list of references raises
doubts. We advise you to reduce the list of references."

\textbf{We had inadvertently included some references that we had read through in our research, but not directly referenced in the paper. We have removed extraneous references and cleaned up the reference section.}

\subsection{Reviewer 2}

\textbf{NOTE TO REVIEWER: We have re-written and better organized the related work and experiments/results sections.}

\noindent(1) ``EEG signal processing has known a huge interest during
the last decade, several models, processing and training
methodologies dedicated to EEG have been published. The
authors give a list of a part of the existing models but
did not analyze the related work to point out the context
in which this work is inserted. Moreover, several papers
concerning the use of transfer learning for EEG processing
(and other fields) are listed in the references but not
cited in the paper, have these references been used for
this paper? Related work section should be revised
including transfer learning approach for EEG."

\textbf{The rewrite of the related work section covers this.}

\noindent(2) ``In the dataset subsection, the employed dataset and the
data split with and without fine-tuning is presented. The
reviewer suspects that an inversion of references has been
made and that the reference [91] (not presenting an EEG
dataset) has been inverted with [1]. For the clarity of the
review, the reviewer will consider [1] when they will
mention the dataset. Moreover, as mentioned several times
in the paper, EEGs are signals that tend to be affected by
noise, however, no pre-processing steps are described? Have
the authors considered a specific signal pre-processing:
signal filtering, artefact removal method, etc? The
duration and sample frequency of the EEG signals are not
given which makes the paper very difficult to reproduce.
Finally, in the paper a study on the number of considered
electrodes has been made, however, the chosen 8/12 among
the 64 available is not mentioned in the paper either."

 \textbf{The reviewer is correct that the reference has been inverted. We have added the citation suggested by the reviewer as well as an additional citation by the same author which addresses the dataset in more detail. This is referenced in Sec. III-A. In this same section, we also mention:  ``For each trial, 1 second of EEG was collected at a 256 Hz sampling rate. Trials were
then filtered using a bandpass filter. In our experiments, we
use these filtered trials as is, with no re-sampling. While the
images were shown, EEG measurements were collected using
64 scalp electrodes (channels) with a standard 10/20 extended
spatial configuration [41]. Of the 64 channels, four serve as
reference and/or ground, so we conducted our experiments
using only the 60 non-reference channels or subsets thereof
according to the same 10/20 configuration.''}


\noindent(3) ``The authors proposed a dataset split based on subject
independent validation (i.e. training with N-i participants
and doing the test on the i remaining). However, it seems
that they only consider one split but did not re-iterate
the process to have a fair distribution of the participant
in each set (in the leave one subject cross-validation,
i.e. i=1, the process is reiterated for each participant
and the mean cross-validation for all the participant is
computed), this could affect the results depending on the
considered participant."

\textbf{The discussion of splits is clarified in Section III-A. The reviewer has a legitimate point that statistical aggregation using a leave one out regime does yield more robust results. However, the effect on results is specifically a concern with smaller numbers of subjects + trials. The dataset we utilize is relatively large compared to other datasets in the EEG space along both these veins and given that we utilized the same splits across experiments with consistent random seeds for weight initializations for our CNN model, the benchmarks offer actionable insights. Moreover, in setting the stage for future work with larger scale datasets, leave one out becomes an increasingly costly benchmark (e.g., leave one out is not used in large-scale computer vision evaluations b/c it is prohibitively expensive).} 

\noindent(4) 11The proposed ML and DL models seem straightforward
compared to existing works, is there any reason for this?
The proposed custom architecture by the authors is composed
of three 1D convolutions followed by a feed-forward neural
network, is there a particular choice for this
architecture? Why did not the authors consider channel-wise
convolution as it has been seen in more recent works [2]?" 

\textbf{We now elaborate in detail on the choice + rationale for architecture in Sec. III-B. We also reference the EEGNET paper, mentioning: ``A number of changes/refinements could be integrated, e.g., channel-wise
convolutions from [26], which could be an interesting future study. We note that we do not conduct a thorough architectural exploration in this paper, since the aim of our present study is to explore cross-subject transfer learning rather than perform detailed architectural comparisons".}

\noindent(5) ``It exists various approaches for transfer learning in
EEG [3], however in this work the authors only consider the
naive model fine-tuning. Is there any reason to choose this
method?"

\textbf{While it is correct that there are multiple approaches for transfer learning in EEG, we specifically focus on deep transfer learning on filtered EEG signals (i.e., no direct feature engineering), which already narrows down this subset. Within the broader deep learning literature, while there are an abundance of transfer learning methods, our approaches are relatively ubiquitous. In this paper, we are specifically interested in exploring the viability of cross-subject transfer. Exploring additional transfer learning techniques is a logical follow-up for future work.}

\noindent(6) ``In the experiments section, the authors refer to
results that are not written in the paper and the proposed
figure showing the results are too small to be analysed.
The fact that \textit{'We show a relevant subset of typical results
as it's not feasible to display all 72 related charts in
this paper'} is not eligible, the results could have been
separated into different subsections presenting the effect
of each modification: considered model, number of
electrodes, weight freezing, fine-tuning partition etc. The
results section has to be reworked."

\textbf{We agree that the experiments section in the originally submitted manuscript could have been clearer. Consequently, we re-wrote the entire section and specifically selected relevant results and added some results in tabular form.}

\subsection{Reviewer 3}

\noindent (1) ``The quality of images should be improved. The text is
not readable."

\textbf{The image quality has been improved and the images have been enlarged.}

\noindent(2) ``The view of an ideal BCI classifier does not seem
realistic. Not only the human brain is an ever-changing
model, but the EEG data collected from an individual during
a particular activity can vary because of emotions, mental
state, thoughts, etc. Finding a classifier that will be
all-encompassing of EEG data ever generated for an activity
does not seem feasible."

\textbf{We acknowledge that an “ideal BCI classifier” may never be attainable. However, we ultimately removed discussion of an “ideal BCI classifier”, as we believe that this distracts from the tangible results that this paper presents.}

\noindent (3) ``The statement (section III.A), \textit{'publicly available EEG
datasets of sufficient size and labeling that meets our
needs for this study'}, is very vague."

\textbf{Good point. We have elaborated on dataset requirements in Sec. III-A.
``However, training DL architectures on direct EEG data (as opposed to featurized data) requires additional labeled data and model regularization to avoid over-fitting [19]. This is an inherent limitation on performance achievable by current DL BCI classifiers"}

\noindent (4) ``Short hand notation should be used only after full forms
have been stated, eg, HR/LR"

\textbf{We have replace “HR/LR” with “High-Risk/Low-Risk”.}

\noindent (5) ``Dataset should be explained in brief. Mean age and
gender of participants, type of electrodes, device name,
tasks, duration for which data was collected, was any
preprocessing done?, etc."

\textbf{We explain the dataset in further detail in Sec. III-A and how we split it specifically for our experiments. We also provide additional citations which detail the dataset and collection process.}

\noindent (6) `` \textit{'Most BCI classifiers require
more data than what is typically provided to train
against.'} Support this with references."

\textbf{We have removed this phrasing and mention several times throughout the paper that BCI datasets are relatively small in the context of machine learning approaches and specifically deep learning approaches. Specifically, see Sec. 1 and Sec III-A.}

\noindent (7) ``What are T1, T2 and T3? Explain clearly."

\textbf{Dataset splits are now discussed in detail in Sec. III-A.}

\noindent (8) ``How was the selection of trials per subject for fine
tuning done? Was it random?"

\textbf{This is now discussed in Sec. III-A, Scenario 1 and III-A, Scenario 2.}

\noindent (9) ``\textit{'datasets of sufficient
size and labeling that meets our needs for this study'}.
This statement is vague and should be explained. How would
you quantify \textit{'needs for this study'}?"


\textbf{We have substantially re-written portions of this paper, consequently removing this vague phrasing. Please see Sec. I and Sec. II-A for discussion.}


\noindent (10) ``\textit{'Within each test, we started the test
with 8 channels, then 12 channels, and finally 60
channels'}. How were the channels selected? Was it random or
channels from nearby areas included, etc?"

\textbf{Chanel sampling/subsampling was conducted according to the 10/20 spatial configuration. We mention in Sec. III-A:``Of the 64 channels, four serve as reference and/or ground, so we conducted our experiments using only the 60 non-reference channels or subsets thereof according to the same 10/20 configuration."}

\noindent (11) ``The statement, \textit{'Selected channels correspond to typical
BCI configurations'} is very vague. Please elaborate."

\textbf{Please see above.}

\noindent (12) ``\textit{'One paper saw similar results on this type of EP
(P300), but surmised it was due to applying a prior spatial filter to
the data [96]. The authors’ conclusion is likely inaccurate, since our data has no such filter applied to it'}. Did the paper use the same dataset? If not then this statement does not seem fair."

\textbf{Out of fairness, we removed this assertion.}

\noindent (13) ``Many previous studies show that ensemble models perform
better than classical machine learning models for EEG. They
also show that deep learningmodels like 1D-CNN, LSTM
perform better with it than machine learning. The
contribution of the paper does not seem novel on that
front"

\textbf{This paper specifically addresses cross-subject deep transfer learning, but as the dataset and dataset configuration that we use have not been benchmarked in other literature, it is important to establish the relative performance of our approach with respect to other common ML classifiers including our tested ensemble methods (gradient boosting and random forests). We are encouraged that our findings are consistent with other literature in the field.}

\noindent(14) ``It does not seem fair to use more data for training for
transfer learning partition."

\textbf{We assume that this comment is in reference to the incorporation of the validation set from Scenario 1 into the training set of Scenario 2 (see the revised Fig. 1). This in no way biases the presented results, as it only affects the Scenario 2 experiments, which are consistent throughout and separated from Scenario 1 results.}

\noindent (15) ``\textit{'however, as the amount of data
increases other more robust classifiers catch up and then
surpass the performance of LDA.'} If other classifiers are
more robust than LDA then what is the reason for comparison
with LDA?"

\textbf{We have changed the phrasing of this within the paper. See Sec. IV-A. We compare with LDA as LDA is a commonly used classifer in the BCI space.}
\end{small}
